The Power of Types: Exploring the Impact of Type Checking on Neural Bug Detection in Dynamically Typed Languages

Motivation: Automated bug detection in dynamically typed languages such as Python is essential for maintaining code quality. The lack of mandatory type annotations in such languages can lead to errors that are challenging to identify early with traditional static analysis tools. Recent progress in deep neural networks has led to increased use of neural bug detectors. In statically typed languages, a type checker is integrated into the compiler and thus taken into consideration when the neural bug detector is designed for these languages. Problem: However, prior studies overlook this aspect during the training and testing of neural bug detectors for dynamically typed languages. When an optional type checker is used, assessing existing neural bug detectors on bugs easily detectable by type checkers may impact their performance estimation. Moreover, including these bugs in the training set of neural bug detectors can shift their detection focus toward the wrong type of bugs. Contribution: We explore the impact of type checking on various neural bug detectors for variable misuse bugs, a common type targeted by neural bug detectors. Existing synthetic and real-world datasets are type-checked to evaluate the prevalence of type-related bugs. Then, we investigate how type-related bugs influence the training and testing of the neural bug detectors. Findings: Our findings indicate that existing bug detection datasets contain a significant proportion of type-related bugs. Building on this insight, we discover integrating the neural bug detector with a type checker can be beneficial, especially when the code is annotated with types. Further investigation reveals neural bug detectors perform better on type-related bugs than other bugs. Moreover, removing type-related bugs from the training data helps improve neural bug detectors' ability to identify bugs beyond the scope of type checkers.

==> initial-version/sections/background.tex <==
\section{Background}
% \subsection{Traditional static analyzers for automated bug detection}
% % Automated bug detection plays a crucial role in software engineering, enabling early identification of bugs during the software development cycle. Traditionally, this task has relied extensively on static analysis to interpret the semantics of the source code \cite{aftandilian2012building,calcagno2015moving,hovemeyer2004finding}. Such tools often demand considerable manual effort to establish patterns for specific bugs \cite{habib2018many}. Moreover, the latest static-based tools are capable of detecting only specific types of bugs~\cite{zz,xx}.

% Automatic bug detection targets to flag erroneous programs in a project and localize the bugs. Traditional bug detection techniques typically involve a static analyzer and a pre-defined set of bug patterns. Bug detection tools are widely used in practice. For example, Error Prone \cite{aftandilian2012building}, PMD \cite{copeland2005pmd}, or Infer \cite{calcagno2015moving} are popular static analyzers to detect bugs in statically typed programming languages like Java, while Pylint \cite{thenault2001pylint} and Pyflakes \cite{Pyflakes} are widely used for Python. Static analyzers can detect specific types of bugs based on the execution semantics  of the program, while they  typically ignore other useful information present in the source code such as the intended meaning of the variable names, comments, etc. 

%\todo{paragraph for NN}
% Recent advancements in machine learning have sparked increased interest in employing neural networks to identify a variety of bugs without the need for explicitly defining bug patterns \cite{habib2019neural}. These solutions typically focus on addressing bug types that elude traditional rule-based static analyzers (e.g., variable misuse~\cite{allamanis2017learning} or binary operator bugs~\cite{troshin2022probing}). Consequently, they are considered complementary tools to be used alongside these traditional analyzers.

%However, when training and testing these neural models, the use of these traditional analyzers are not taken into account ... the bugs detected by these traditional methods are not 
\label{sec:background}
\subsection{Type checking for Python}
Type checkers are a category of bug detectors based on static analysis targeting to identify defects using the types of variables. These type checkers are typically integrated into the compiler of statically typed languages and can be used as external tools in dynamically typed languages \cite{rak2020python}. %Due to its widespread popularity and ease of integration into the development process, this paper focuses on type checkers as static type bug detectors. 

Python is a dynamically typed language thus it only determines the type of a variable at runtime. However, starting with Python 3.5, optional type annotations are introduced to both help the developer understand the code better and enable static type checkers to detect type-related bugs \cite{PEP484}. 

There are two type-checking frameworks for type checkers in Python: gradual typing and type inference \cite{rak2020python}. Many popular type checkers, such as \emph{mypy} \cite{mypy}, operate on the principles of \emph{gradual typing}, a framework that detects inconsistencies in types based on annotated types in the program \cite{siek2007gradual}. However, gradual typing often assigns \emph{unknown} types to unannotated variables, which limits its ability to detect type-related bugs in the absence of type annotations. \emph{Type inference} is a technique similar to gradual typing but with a key distinction: it infers types for variables even without explicit type annotation in the code, thereby enabling the detection of a broader spectrum of type-related bugs. Given that Python datasets used for bug detection often lack type annotations, this paper uses \texttt{pytype} \cite{pytype}, a popular open-source type inference-based type checker.

Recent advancements have seen deep learning-based approaches being applied to type inference in Python. The core concept involves using neural networks to learn typing patterns implicitly in programs, subsequently annotating variables based on these patterns. Tools such as DeepTyper \cite{hellendoorn2018deep} and Typilus \cite{allamanis2020typilus} have demonstrated the ability to infer complex types that are difficult to infer by traditional methods. However, these tools have not yet been widely adopted in practice due to their high computational demands and the challenges in explaining the rationale behind their type inferences. Thus, we do not consider these types of inference tools in this paper.

\subsection{Variable misuse bugs}

A variable misuse bug occurs when a developer unintentionally uses an incorrect variable. \autoref{lst:codeExp} shows an example of a variable misuse bug. In this snippet, the developer mistakenly uses the variable \texttt{first} instead of \texttt{last} in line 8, \texttt{if (assn[1]!=first[1]):}.

\begin{lstlisting}[language=python, caption={Example synthetic faulty program extracted from a Python variable misuse dataset. Incorrect variable use location is bold and colored in red}, label={lst:codeExp}, numbers=left]
    def take_last_assignment(source):
        |\textbf{first}|=True
        last=None
        for assn in source:
            if |\textbf{first}|:
                last=assn
                |\textbf{first}|=False
            if (assn[1]!=|\textcolor{red}{\textbf{first}}|[1]):
                (yield last)
            last=assn
        if (last is not None):
            (yield last)
\end{lstlisting}
%\textit{e.g.,} she uses a variable before it is defined, or uses a different variable than the intended one

Such bugs are widespread in SE practice. For instance, 12\% of the bugs in the ManySStuBs4J corpus are variable misuse bugs\cite{karampatsis2020often}, while around 6\% of build errors in Google engineering systems can be attributed to variable misuse bugs \cite{allamanis2022graph}. In open-source projects, Allamanis et al. \cite{allamanis2017learning} also find variable misuse bugs in RavenDB, a popular NoSQL database.

In this paper, we exclusively focus on variable misuse bugs due to their prevalence in SE practice, and because they are commonly targeted by neural bug detectors~\cite{VasicKMBS19,allamanis2017learning, hellendoorn2019global,troshin2022probing}. Furthermore, some of these bugs can potentially be caught by a type checker, which makes this kind of bugs a good candidate for investigating neural bug detectors in a practical SE setting. Furthermore, we focus on detecting a single bug in a code snippet, which is a common assumption in the literature of neural bug detection \cite{VasicKMBS19, hellendoorn2019global,troshin2022probing}.

\subsection{Neural bug detectors for variable misuse}

% This paper focuses on single-bug detection tasks where the code snippet contains at most one faulty location. 

This section overviews the task of detecting variable misuse, and the neural network architectures used to tackle such task.

\subsubsection{Task}
Given a program, a bug detector targeting variable misuse bugs produces two outputs: (1) a decision on whether the program contains such a bug and (2) the location of the variable misuse, if the program contains a bug. Formally, given a bug detector $\mathfrak{D}$ and a program (function) $P$, the output of the bug detector can be represented as $\mathfrak{D}(P) = (d, l)$, where $d$ is a Boolean value indicating whether the program has a bug or not, and $l$ represents the location of the bug when $d = \texttt{true}$. 

% We focus on the two most popular neural network architectures for bug detection: transformers and graph neural networks (GNNs). We also discuss the two main representations of programs: source code and program graphs.

% The two most popular neural network architectures for bug detection are transformers and graph neural networks (GNNs).

%\subsubsection{Program representation} 
% Transformers and GNNs process distinct types of input while a program can also be represented in different formats. In this paper, we focus on programs with a single function with two main representations of programs: source code and program graphs.

%\textbf{Source code.} 
%The most straightforward approach to represent a program is to use its source code. For sequence neural networks like transformers, the program's source code is split into a sequence of tokens. This token sequence is then fed into the neural network to generate a prediction. Nevertheless, the inherent complexity of information within the source code often exceeds what can be captured through simple textual representation, limiting the model's ability to fully understand the semantics of programs.  

%\textbf{Program graphs.}
%Alternatively, compilers often translate the source code into graphs that incorporate additional information like control flow and data flow extracted from the code. In this case, the node of the graph typically represents a program element (e.g., a variable, a function, or a statement) and the edges represent the relationships between these elements such as use definition or control flow. These program graphs aim to capture the complex aspects of source code more effectively \cite{allamanis2017learning}. 

% While graph neural networks are typically for such graphs \cite{kipf2016semi}, transformers are also adapted to work with program graphs \cite{hellendoorn2019global}.


\subsubsection{Architectures}
The three prevalent neural network architectures used to tackle the variable misuse task are transformers, graph neural networks (GNN), and hybrid approaches.

% \todo{A special token for deciding no bug}
\noindent\textbf{Transformers} represent a class of neural networks that process inputs as sequences of tokens, leveraging a multi-head attention mechanism to capture global relationships within these tokens \cite{vaswani2017attention}. 
% Formally, the attention mechanism considered three matrices $Q, K, V$ for all token $t$ and calculated the result of a attention head using
% \begin{equation}
%     \label{equ:attention}
%     Attention(Q, K, V) = softmax(\frac{QK^T}{\sqrt{d_k}})V
% \end{equation}
% Finally, multiple attention heads can be calculated to capture different aspects of the input data. Results from different attention heads are then concatenated to form the final result. 
In this case, the programs are represented as a sequence of tokens and the output bug location ($l$) corresponds to the token that causes the bug. While it is possible to train transformers from scratch with randomly initialized weights, they are typically pre-trained on extensive data corpora and subsequently fine-tuned for specific tasks. These pre-trained models are known as pre-trained language models. This paper focuses on encoder-only language models as they are predominantly used in fine-tuning for classification problems~\cite{lin2022survey}. Specifically, in our experiments, we use CodeBERT \cite{feng2020codebert}, GraphCodeBERT \cite{guo2020graphcodebert}, and UnixCoder~\cite{guo2022unixcoder}, all of which are pre-trained models specialized in source code.

\noindent\textbf{Graph neural networks (GNNs)} process graphs with both structural and feature information \cite{kipf2016semi}. 
Hence, the programs are depicted as program graphs~\cite{allamanis2017learning}, encompassing details concerning control flows (\textit{e.g.,} branching and loops) and data flows (\textit{e.g.,}, last read and last write of a variable). Consequently, the output bug location ($l$) corresponds to the node representing the token responsible for the bug. The most frequently used GNNs for bug detection are gated graph neural networks (GGNN)~\cite{allamanis2017learning} which use a gated recurrent unit (GRU) \cite{cho2014properties} to perform the neighbor aggregation~\cite{li2015gated}. 
%Unlike traditional graph convolutional networks where the graph can only contain one edge type, GGNNs are tailored to handle graphs with multiple edges types through a message passing mechanism specific to each edge type. Furthermore, a gated recurrent unit (GRU) \cite{cho2014properties} is used to update a node representation from the aggregation of its neighbors. 

\noindent\textbf{Hybrid approaches}
combine both transformer and graph neural network approaches. In our study, we explore the Graph-Relational Embedding Attention Transformer (GREAT) architecture proposed by Hellendoorn et al.~\cite{hellendoorn2019global}. GREAT harnesses the capabilities of both transformers and GNNs by enhancing the attention mechanism with biases for different relationship types. The central concept behind GREAT is incorporating edge information into the transformer architecture by using a \textit{relation type bias} term in the attention computation.


%Transformer-based models effectively consider global relations among tokens yet do not explicitly identify the types of these relations, particularly those in the program graph. Conversely, GNNs recognize the types of relationships between tokens but are limited to capturing local relations from the program graph. The Graph-Relational Embedding Attention Transformer (GREAT) \cite{hellendoorn2019global} combines the strength of both Transformers and GNNs by refining the attention mechanism through the inclusion of a bias for each relationship type. This approach introduces a \emph{relation type bias} for pairs of tokens connected by an edge in the program graph, allowing the neural network to simultaneously account for global relations and specific relation types outlined in the program graph. 

% This approach computes a bias value $B_{ij}=W_r^Tr+b_r$ for tokens $i, j$ connected by a type $r$ within the program graph, assigning zero otherwise. Here $W_r, b_r$ and $r$ represent learnable embeddings. When multiple edges connect tokens $i$ and $j$, the corresponding bias values are aggregated. This enhancement is then used to update \autoref{equ:attention} with the bias matrix $B$, as shown in the following equation: 

% \begin{equation}
%     \label{equ:attention}
%     Attention(Q, K, V) = softmax(\frac{(Q+B)K^T}{\sqrt{d_k}})V
% \end{equation}

%For variable misuse, these models are trained as token classification task with two main objectives: (1) classify the presence of bugs in code using a special token in the code sequence and (2) identify the token representing the bug location within the code \cite{VasicKMBS19}. 

% \subsection{Training datasets for variable misuse bugs}
% \todo[inline]{Maybe remove}
% The challenge of obtaining real-world bugs for neural network training has led many researchers to use synthetically generated bugs for training neural bug detectors \cite{hellendoorn2019global,habib2019neural}. Subsequently, these detectors are assessed using both synthetic and real-world bugs \cite{he2022distribution,richter2023train}.

% %In our study, we concentrate on synthetic bugs created by randomly mutating correct programs. 
% Although there exist more advanced techniques for generating synthetic bugs \cite{richter2022learning,patra2021semantic}, they are not yet widely adopted in the training of neural bug detectors. Therefore, in our experiments, we train the neural bug detectors using a synthetically generated dataset for variable misuse proposed previously, and we evaluate the models using both the corresponding test split of the synthetic dataset and real-world datasets.

%To generate synthetic variable misuse bugs, we first process the program to identify all variables declared within the scope. Subsequently, a variable usage is randomly selected and replaced with another variable from within the same scope. Throughout this paper, we define the scope of variable misuse bugs as a single function.
 

% This paper focuses on one type of synthetic bug: \emph{variable misuse} \cite{hellendoorn2019global,habib2019neural}.

% \textbf{Variable Misuse.}
% In variable misuse, the program contains one location where the variable is used in an undesired way. For example, a variable is used before it is defined, or a different variable is used than the intended one. 


% However, variables in Python typically do not have statically annotated types. Therefore,  the type information of variables is not considered when generating synthetic variable misuse bugs \cite{hellendoorn2019global}. 

% \textbf{Operand Swapping.}
% The operand swapping bug occurs when the program contains one non-commutative operator whiles its operands are swapped. For example, the program contains the expression \texttt{a - b} but the operands are swapped to \texttt{b - a}. When generating synthetic operand swapping bugs, one non-commutative operator is randomly selected and its operands are swapped \cite{kanade2020learning}.
 

%\subsection{Static Analysis and Neural Bug Detectors}

==> initial-version/sections/conclusion.tex <==
\section{Conclusion and future work}
\label{sec:conclusion}

In this study, we explore the impact of type checking on automated bug detection using neural networks, focusing on variable misuse errors. We found that over 19\% of synthetic bugs and 5\% of real-world bugs in datasets used for neural bug detectors can be identified by a type checker without the need for explicit type annotations. Through experiments with various neural bug detectors, we find that the benefits of type checking are most pronounced when prioritizing bug detection over reducing false alarms. When the neural bug detectors are used together with a type checker, it has been observed that type-related bugs lead to an overly optimistic evaluation. Finally, we discover that excluding these type-related bugs from training can enhance the bug detection capabilities of the neural bug detectors while reducing their precision. As a result, the decision to exclude type-related bugs from training depends on whether the priority of the bug detector is on bug identification or false alarm minimization. 

We plan to extend the work from two aspects. First, the impact of type checking on dynamically typed languages beyond Python and other types of bugs can be investigated. Then, feedback from the type checkers can be used with the recent learning-based synthetic bug generation strategy to further improve the performance of neural bug detectors. 


% the output of the type checker can be used to refine the synthetic bug generation strategy to potentially improve the performance of neural bug detectors. 

==> initial-version/sections/discussion.tex <==
\section{Discussion}
\label{sec:discusssion}

\subsection{Key implications}
In this paper, we demonstrate synthetic datasets for Python variable misuse contain a significant portion of type-related bugs. Furthermore, we conduct systematic experiments to evaluate the impact of type-related bugs on the training and evaluation of neural bug detectors. Based on the observations, several implications are identified when using neural bug detectors for dynamically typed languages. 

%Taking the practical SE scenario into consideration, while a type checker is integrated into the development process, we evaluate the impact of these type-related bugs on both evaluation and training of the neural bug detectors. 
\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
\textbf{Takeaway 1}: Neural bug detectors are recommended to be used together with static type checkers for dynamically typed languages when bug detection is key.
\end{tcolorbox}

Many existing studies have demonstrated that type checkers can help identify bugs in dynamically typed languages when manual type annotation is provided \cite{khan2021empirical,gao2017type}. Our study builds upon these findings, revealing that type checkers are capable of detecting a significant proportion of real-world bugs, up to 5.72\%, even in the absence of explicit type annotations.

Based on this observation, we assess the combined use of type checkers and neural bug detectors. Analysis of this assessment indicates that when the priority is bug identification over reducing false positives, incorporating type checkers is recommended to ensure early bug detection.

% We demonstrate that the neural bug detectors perform better at identifying and localizing type-related bugs over others. However, none of the bug detectors we evaluated in this study are able to identify all type-related bugs detected by the type checker, especially real-world bugs. This finding indicates that even though currently neural bug detectors are able to detect a wide range of bugs, they cannot replace the role of type checkers in the development process. As also suggested by previous work \cite{richter2022neural}, neural bug detectors should be used together with static type checkers.

% We suspect these projects may not have used type checkers in the development process. If a type checker is used, these bugs can easily be identified and fixed before they are included into the codebase. 

% \begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
% \textbf{Takeaway 2}: Neural type detectors are recommended to be used together with static type checkers.
% \end{tcolorbox}



\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
\textbf{Takeaway 2}: When evaluating neural bug detectors, type-related bugs and other bugs should be evaluated separately. 
\end{tcolorbox}

Existing assessments of neural bug detectors typically combine all bug types into a unified dataset. Our findings reveal that excluding type-related bugs from the evaluation dataset significantly reduces the neural bug detectors' performance. Therefore, to accurately estimate the effectiveness of neural bug detectors in conjunction with a type checker, removal of these type-related bugs from the evaluation is necessary. Conversely, if the aim is to evaluate the neural bug detector's stand-alone performance, a more detailed bug categorization should be used to comprehensively understand their capabilities.

% However, we find that the type of bugs in the dataset can significantly influence the performance of neural bug detectors. In order to have a more accurate estimation of the performance, especially for practical purposes, the performance measures on type-related bugs and other bugs should be separated. Furthermore, more fine-grained categorization of bugs should be considered to obtain a more comprehensive understanding of the performance of neural bug detectors.

% \begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
% \textbf{Takeaway 3}: When building a neural bug detector from scratch, fine-tuning methods should be favored compared to full training.
% \end{tcolorbox}

% Similar to previous work \cite{he2022distribution}, we find that the neural bug detectors trained with a pre-training language model and fine-tuning perform better than the ones with full training. This is especially the case when these models are evaluated on real-world bugs, showing the difference in generalizability. Such improvement is expected as the pre-trained language models have already gained information from a large amount of pre-training code corpus, which is beneficial for the generalization of the model.  

\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
\textbf{Takeaway 3}: When training a neural bug detector to complement type checkers, eliminating type-related bugs from the training datasets enhances the neural model's ability to detect non-type-related bugs. However, this refinement often leads to a decrease in precision.

%then type-related bugs should be removed from the training data. 
\end{tcolorbox}
Excluding type-related bugs from datasets during the training phase results in general improvements in recall for all neural bug detectors within both synthetic and real-world datasets. However, this improvement in recall comes at the cost of a reduction in precision. Thus, the decision to exclude these bugs from training depends on the specific goal of the bug detector. If the emphasis is on detecting more bugs rather than minimizing false positives, then eliminating type-related bugs during training is advantageous.

%This trend is consistent even in real-world programs, suggesting an improvement strategy for neural bug detectors. Specifically, when the objective is to identify bugs beyond the scope of a type checker, it is advantageous to omit type-related bugs from the training dataset.

% When training with dataset filtering the type-related bugs, a general improvement is observed in recall for all neural bug detectors in the synthetic dataset. Even though the precision slightly drops, the joint performance improves since the improvement in recall is more significant than the decrease in precision. This finding also extends to the real-world dataset. This finding indicates that when the purpose of the neural bug detector is to focus on detecting bugs beyond the scope of a type checker, the type-related bugs should be removed from training.


% Even though the performance on correct program recall is generally negative impacted, the impact is not significant and is smaller compared to the improvement in the localization accuracy. This finding indicates that when the purpose of the neural bug detector is to focus on detecting bugs beyond the scope of a type checker, the type-related bugs should be removed from training.

\subsection{Threats to validity}
\paragraph{Internal validity}
Training and fine-tuning of neural networks can be sensitive to the choice of hyperparameters. We mitigate this issue by reusing hyperparameters from previous work \cite{hellendoorn2019global}. Furthermore, for the same reason, we use the same hyperparameters for the same model architecture when training with the full and filtered dataset. Moreover, the training process can be non-deterministic and, due to the cost of training, we only used one random seed for each setting. To mitigate this issue, we experimented with multiple different neural network architectures and training paradigms. %and found consistent results across all of them.
%This issue is mitigated by training models with the same random seed across all settings

When identifying type-related bugs in the datasets, we do not add any manual type annotations to the code. Typically, type checkers can identify more bugs when type annotation is provided \cite{khan2021empirical}. As a result, the portion of type-related bugs identified in the dataset is a lower bound for the actual portion. Furthermore, when evaluating the impact of type-related bugs in the training data, we consider oversampling the existing type-related bugs to keep the dataset balanced. Such a strategy provides significant improvement in recall. Another approach could have been to generate more synthetic bugs while filtering type-related bugs. We suspect that such an approach will further improve the performance and it is left as future work.

\paragraph{External validity}
%The synthetic dataset used in this study is generated from a single dataset. While the dataset already covers a wide range of popular open-source project, we further mitigate this concern by evaluating the performance on two real-world datasets built both using GitHub an PyPI. 
This paper exclusively concentrates on Python due to the limited availability of variable misuse datasets for other dynamically typed languages. Consequently, the insights drawn from this study might not be directly transferable to other dynamically typed languages. We defer the exploration of such intriguing avenues to future research.
Additionally, we rely solely on one type checker to detect and classify type-related bugs. Alternative type checkers may yield varying percentages or categorizations for these bugs. To address this concern, we chose \texttt{pytype}, a widely used type checker developed by Google and consistently updated.

%A popular type-inference based type check, \textit{pytype} is used to identify and categorize type-related bugs. Other type checkers may identify different percentage or assign different categories to these bugs. To systematically evaluate the impact of type-related bugs, a wide range of neural bug detectors are evaluated. Finally, we focus on one of the most popular dynamically typed language, Python. While the finding in this study may also be applicable to other dynamically typed languages, we leave it as a future work.

\paragraph{Construct validity}


Selecting appropriate performance metrics to evaluate performance in the variable misuse task presents a potential threat to validity. To tackle this concern, we use standard metrics for classification by considering bug detection as a classification problem. These metrics cover existing metrics used for neural bug detectors such as correct program recall and location accuracy~\cite{hellendoorn2019global,VasicKMBS19}. 

In assessing the joint effectiveness of neural bug detectors, we employed the \fbeta{} score as our metric. The choice of $\beta$ values is tailored to balance the emphasis between identifying bugs and minimizing false alarms. To address variability in performance, we present results across a spectrum of $\beta$ values during pipeline performance evaluation. Furthermore, we select two $\beta$ values to represent different scenarios in our analysis of the influence of type-related bugs on training.


==> initial-version/sections/evaluation.tex <==
\section{Effect of Type Checking}

\subsection{Motivation}


%Though type-related errors exist in both synthetic and real-world datasets, the former contains a much higher proportion of such bugs. 

In scenarios where a type checker is employed, neural bug detectors are expected to focus on bugs not detectable by the type checker. Thus, to offer recommendations for deploying neural bug detectors alongside a type checker, it's crucial to comprehend the impact of type-related bugs on the training and testing of these neural systems. As a result, we aim to address the following two research questions:


%In real world setting when a type checker is deployed in development, the type-related bugs are often caught before by the type checker 

%they are pushed into the code base by a type checker. Thus, it is important to understand how type-related errors influence the training and testing of the the neural bug detectors. Specifically, we investigate the following two research questions:

%This section presents our experiment results demonstrating the effect of type-related bugs on the performance of these neural bug detectors in both evaluation and training. Specifically, we investigate the following two research questions:

\begin{itemize}
    \item \textbf{RQ2:} How do type-related bugs influence the evaluation of neural bug detectors?
    \item \textbf{RQ3:} How do type-related bugs influence the training of neural bug detectors?
\end{itemize}


\subsection{Experiment Setup}
In this section, we introduce the neural networks used in the neural bug detectors in our experiments. This is followed by datasets and evaluation metrics we used to investigate the research questions. 


\begin{table}[tb]
    \centering
    \caption{Bug Detection Neural Networks}
    \begin{tabular}{cccc}
    \hline
    \textsc{Model} & \textsc{Architecture} & \textsc{Training strategy} \\
    \hline
    GGNN \cite{allamanis2017learning} & GNN & From scratch \\
    % \hline
    % 6-layer transformer \cite{hellendoorn2019global} & Transformer & Full \\

    CodeBERT \cite{feng2020codebert} & Transformer & Fine-tuning \\

    GraphCodeBERT \cite{guo2020graphcodebert} & Transformer & Fine-tuning \\

    UnixCoder \cite{guo2022unixcoder} & Transformer & Fine-tuning \\

    GREAT \cite{hellendoorn2019global} & Hybrid & From scratch \\
    \hline
    \end{tabular}
    \label{tab:models}
\end{table}

\subsubsection{Neural bug detectors}


The first column of \autoref{tab:models} displays the neural bug detectors utilized in our experiments. The second column of the same table illustrates the architectures corresponding to each considered model. We cover three widely employed architectures: transformers, GNNs, and hybrid methods. Lastly, the third column denotes whether the model is trained from scratch (\textit{i.e.,} initialized with random weights) or fine-tuned (\textit{i.e.,} initialized with a pre-trained checkpoint).

%In this paper, we focus on three main architectures of neural networks: graph neural networks, transformers, and hybrid methods. Furthermore, they can also be categorized by the training strategy: full training or fine-tuning. \autoref{tab:models} presents the neural networks used in our experiments.

%When fine-tuning a pre-trained model, we follow previous work \cite{troshin2022probing} by appending a classification layer to the pre-trained model and fine-tuning the entire model. For the full training models, we adapt the implementation from previous work \cite{hellendoorn2019global}

\subsubsection{Datasets}


We adopt the methodology established in prior studies concerning training with a synthetic dataset and assessed using both the synthetic test split from the same dataset and real-world datasets~\cite{hellendoorn2019global,habib2019neural,he2022distribution,richter2023train}. Specifically, we select the Synthetic 1 dataset as our training dataset because of its larger volume of data.
%For detecting variable misuse task, we use the training split of the \textit{Synthetic 1} due to its larger amount of data and its distribution of type-related errors is closely aligned with that of real-world scenarios. Subsequently, we evaluate the trained models also on the test split of the dataset.

The trained neural bug detectors are also evaluated in the real world in both real-world datasets: \emph{Real-Py150} and \emph{Real-PyPI}. For the \emph{Real-Py150} dataset, we include the correct programs from the test splits as well as faulty programs from all splits. All processed variable misuse bugs from \emph{Real-PyPI} dataset are also included in the evaluation. 

%\textbf{Data leakage check}
Since the real-world datasets are constructed independently from the \emph{Synthetic 1} dataset, some of the real-world bug programs may also appear in the training set of \emph{Synthetic 1}. To avoid such data leakage issues, all potential duplicated samples are excluded from the datasets from evaluation. Specifically, we use the metadata of each sample as a heuristic and remove all program samples that are from the same file in the same repository and have the same function signature as any samples from the synthetic training set. \todo[inline]{how many are removed - does the number of real bugs stated earlier include the duplicates?}

% We perform data leakage check on the \textit{VarMisuseReal} dataset and found it does not contain any files from the repositories as the synthetic dataset. Thus, we include all faulty programs from this dataset and randomly sample the same number of correct programs to build a balanced real world test set.

\subsubsection{Metrics}
Following previous work \cite{hellendoorn2019global,habib2019neural}, we use separate metrics for bug classification and localization. First, we measure the \textit{correct program recall} (\textbf{CPR}), which is the recall of a neural bug detector in deciding that a program is free from any bugs. Specifically, given a neural bug detector and a set of \emph{correct} programs $\mathcal{P}_c$, the \textbf{CPR} is defined as:
\begin{equation*}
    CPR(\mathfrak{D}, \mathcal{P}_c) = \frac{|\{p\in\mathcal{P}_c|d_{\mathfrak{D}(p)} = \texttt{false}\}|}{|\mathcal{P}_c|}
\end{equation*}
where $d_{\mathfrak{D}(p)}$ represents the decision of the neural bug detector on the program.

Then, for all the faulty programs, we measure the \textit{location accuracy} (\textbf{LA}) which is the proportion of programs where the model correctly identifies the location of the bug. Let $\mathcal{P}_f$ represent the set of \emph{faulty} programs and $l_p$ represent the location of the bug for the program $p$, \textbf{LA} is defined as follows.
\begin{equation*}
    LA(\mathfrak{D}, \mathcal{P}_f) = \frac{|\{p\in\mathcal{P}_f|d_{\mathfrak{D}(p)} = \texttt{true} \land l_{\mathfrak{D}(p)} = l_p\}|}{|\mathcal{P}_f|}
\end{equation*}
where $l_{\mathfrak{D}(p)}$ represent the bug location of the faulty program $p$ predicted by the neural bug detector.

\chadded{
Finally, to measure the differences in performance of the two settings, we use \emph{ratio change}. Given the performance values of two settings $p_a$ and $p_b$, the ratio change $\Delta$ of $p_b$ with respect to $p_a$ is calculated as follows:
}
\begin{equation*}
    \Delta = \frac{p_b - p_a}{p_a} \times 100
\end{equation*}
\subsubsection{Training settings}
Previous work often trains the neural bug detector with the joint training objective of both bug detection and repair \cite{VasicKMBS19,allamanis2017learning,hellendoorn2019global}. In our preliminary experimentation, we notice that training without the repairing loss results in either similar or degraded performance compared to the joint objective. Consequently, we opt to utilize the joint training objective, as done in previous studies.

When training GGNN and GREAT models, we use the same hyperparameter configurations as in previous work~\cite{hellendoorn2019global} and train for 5, 10, and 12 epochs, respectively. For fine-tuning, we train each model for 1 epoch and use a learning rate of 0.00001 with a learning rate scheduler.

\subsection{RQ2: Evaluation on type-related bugs}
\subsubsection{\todo[inline]{for RQ1, we have these four sections: Motivation, Setup, Approach, and Results. therefore, this should be called Approach to be consistent}Addressing the RQ}
In this section, we evaluate the performance of neural bug detectors on type-related bugs compared to other bugs when trained with a synthetic dataset on the variable misuse task. We divide the evaluation dataset into two groups based on the type checking results in the evaluation samples: type-related bugs and other bugs. We then evaluate the performance of the neural networks on these two groups separately. Furthermore, we measure the impact of the type-related bugs on the overall performance by evaluating all faulty programs and faulty programs filtering type-related ones. We only include the location accuracy as the focus of this experiment is on faulty programs. 

% When performing full training on the models, we use the same hyperparameter configurations as in \cite{hellendoorn2019global} and train for 5, 10 and 12 epochs respectively. For fine-tuning, we train each model for 1 epoch and use a learning rate of 0.00001 with a learning rate scheduler.

% \begin{table*}[tb]
%     \centering
%     \caption{Location Accuracy on all bugs, type-related Bugs, other bugs and the difference between type-related bugs and other bugs for synthetic and real world datasets. The numbers are in percentage.}
%     \begin{tabular}{|c|c|c|c|c||c|c|c|c||c|c|c|c|}
%     \hline
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c||}{Synthetic 1} & \multicolumn{4}{c||}{Synthetic 2} & \multicolumn{4}{c|}{Real} \\
%     \cline{2-13}
%     & \textbf{All} & \textbf{Type Bug} & \textbf{Other bugs} & \textbf{Diff} & \textbf{All} & \textbf{Type Bug} & \textbf{Other bugs} & \textbf{Diff} & \textbf{All} & \textbf{Type Bug} & \textbf{Other bugs} & \textbf{Diff}\\
%     \hline
%     CodeBert & 93.95 & 99.07 & 92.72 & 6.34 & 77.17 & 86.37 & 75.78 & 10.59 & 35.40 & 36.36 & 35.33 & 1.03\\
%     \hline
%     GraphCodeBert & 94.74 & 99.18 & 93.68 & 5.50 & 81.14 & 91.13 & 79.64 & 11.49 & 36.58 & 37.88 & 36.50 & 1.38\\
%     \hline
%     UnixCoder & 94.74 & 99.49 & 93.61 & 5.88 & 74.85 & 85.60 & 73.22 & 12.38 & 36.32 & 37.14 & 36.27 & 0.87\\
%     \hline
%     GGNN & 76.41 & 93.47 & 72.43 & 21.04 & 44.99 & 44.75 & 45.01 & -0.26 & 15.05 & 19.67 & 14.79 & 4.88\\
%     \hline
%     GREAT & 84.31 & 97.00 & 81.34 & 15.65 & 51.26 & 50.87 & 51.29 & -0.43 & 20.73 & 24.59 & 20.52 & 4.07\\
%     \hline
%     Transformer & 67.22 & 75.38 & 65.31 & 10.07 & 41.79 & 40.77 & 41.87 & -1.09 & 8.84 &  9.84 & 8.78 & 1.06 \\
%     \hline
%     \end{tabular}
    
%     \label{tab:location-accuracy}
% \end{table*}

\begin{table*}[tb]
    \centering
    \caption{Location accuracy on type-related bugs and other bugs for synthetic and real-world datasets. The numbers are in percentage. We observe that the neural bug detectors perform better on type-related bugs compared to other bugs in all cases.}
    \begin{tabular}{|c|cc|cc|cc|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{Synthetic} & \multicolumn{2}{c|}{Real-Py150} & \multicolumn{2}{c|}{Real-PyPI} \\
    \cline{2-7}
    & \textbf{Type} & \textbf{Other} & \textbf{Type} & \textbf{Other} & \textbf{Type} & \textbf{Other}\\
    \hline
    CodeBert      & 99.07 & 92.90 & 36.36 & 35.33 & 60.00 & 33.42\\
    GraphCodeBert & 99.34 & 93.78 & 37.88 & 36.50 & 68.00 & 33.29\\
    UnixCoder     & 99.41 & 93.70 & 37.14 & 36.27 & 56.67 & 33.29\\
    GGNN          & 94.07 & 72.64 & 21.43 & 14.76 & 23.68 & 15.18\\
    GREAT         & 97.24 & 81.51 & 28.57 & 20.89 & 50.00 & 20.94\\
    \hline
    \end{tabular}
    
    \label{tab:la-bug-types}
\end{table*}

\begin{table*}[tb]
    \centering
    \caption{Impact of filtering type-related bugs on overall location accuracy. Numbers are in percentage. Type-related bugs make the model performance over-optimistic.}
    \begin{tabular}{|c|ccc|ccc|ccc|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{Synthetic} & \multicolumn{3}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
    \cline{2-10}
    & \textbf{Full} & \textbf{Filtered} & $\Delta$ & \textbf{Full} & \textbf{Filtered} & $\Delta$ & \textbf{Full} & \textbf{Filtered} &$\Delta$\\
    \hline
    CodeBert      & 94.11 & 92.90 & -1.29 & 35.40 & 35.33 & -0.17 & 34.28 & 33.42 & -2.51\\
    GraphCodeBert & 94.91 & 93.82 & -1.15 & 36.58 & 36.50 & -0.23 & 34.41 & 33.29 & -3.26\\
    UnixCoder     & 94.82 & 93.70 & -1.18 & 36.32 & 36.27 & -0.14 & 34.13 & 33.29 & -2.45\\
    GGNN          & 76.78 & 72.64 & -5.39 & 15.17 & 14.76 & -2.68 & 15.54 & 15.18 & -2.34\\
    GREAT         & 84.55 & 81.51 & -3.59 & 21.36 & 20.89 & -2.19 & 22.18 & 20.94 & -5.61\\
    \hline
    \end{tabular}
    
    \label{tab:la-impact}
\end{table*}


\todo{CPR is not mentioned for this research question before}
\begin{table*}[tb]
    \centering
    \caption{Performance of the bug detection pipeline shown in \autoref{fig:motivation}. $\Delta$ shows the percentage change w.r.t. the Full performance in \autoref{tab:la-impact}. The pipeline provides notable improvement to bug localization while marginally reducing correct program recall.\todo[inline]{i don't understand the figures in this table}}
    \begin{tabular}{|c|c:cc:c|cc:c|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
    \cline{2-8}
    & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR} & \textbf{LA} &$\Delta$\\
    \hline
    CodeBert      & 94.15 & -1.55 & 39.22 & 10.80 & -- & 35.58 & 3.77 \\
    GraphCodeBert & 94.61 & -1.55 & 40.31 & 10.20 & -- & 35.45 & 3.01 \\
    UnixCoder     & 94.57 & -1.54 & 40.12 & 10.45 & -- & 35.68 & 4.55 \\
    GGNN          & 91.28 & -1.49 & 19.97 & 31.61 & -- & 18.81 & 21.01 \\
    GREAT         & 87.67 & -1.49 & 25.72 & 20.41 & -- & 24.32 & 9.64 \\
    \hline
    \end{tabular}
    
    \label{tab:pipeline}
\end{table*}

\subsubsection{Results}
\autoref{tab:la-bug-types} shows the location accuracy of the neural bug detectors on type-related bugs (\textbf{Type}) and other bugs (\textbf{Other}) across synthetic and real-world datasets. 


Comparing the performance of the neural bug detectors on synthetic and real-world datasets, we observe that these detectors perform much better on the synthetic datasets compared to the real-world bugs, consistent with previous work~\cite{he2022distribution,allamanis2021self}. This discrepancy can be attributed to the distribution shift between synthetic and real-world bugs~\cite{he2022distribution}. 

Neural bug detectors consistently perform better in identifying type-related bugs, with a difference reaching up to 34.71\% for GraphCodeBert within the \emph{Real-PyPI} dataset. This finding aligns with our observations from the previous research question regarding the trivial nature of type-related bugs.

%indicates that neural bug detectors are indeed better at identifying type-related bugs with are composed of a large portion of trivial errors as shown in \autoref{fig:error-type} 

To check the influence of type-related bugs on the overall performance, \autoref{tab:la-impact} shows the impact of filtering type-related bugs on the overall location accuracy. The ratio of change in the filtered dataset compared to the full dataset is also noted in the table ($\Delta$). Since all neural bug detectors perform better on type-related bugs, we observe that the removal of type-related bugs generally reduces the performance of the neural bug detectors. The highest reduction is observed in the \emph{Real-PyPI} dataset, where the removal of type-related bugs results in a reduction of up to 5.61\% for the GREAT model, even though the type-related bugs only constitute 4\% of the dataset.

%In general, models using a full training strategy tends to bias more towards type-related bugs compared to fine-tuning models. This can be explained by fine-tuning models are already pre-trained with a large amount of code data and thus are less likely to be influenced by the type-related bugs in the training data. At the same time, the impact of type-related bugs on the performance also varies across different datasets, with the highest impact observed in the \emph{Real-PyPI} dataset and the lowest in the \emph{Real-Py150} dataset.

\chadded{
Our observations indicate that, despite being comparatively more effective than other bug types, the performance of neural bug detectors for identifying type-related bugs in real-world datasets remains suboptimal. Therefore, integrating neural bug detectors with a type checker within the pipeline as depicted in \autoref{fig:motivation}, is expected to enhance the performance in bug localization. To evaluate the performance of this integrated pipeline, we conducted experiments using the type checker on the correct programs within the \emph{Real-Py150} dataset. 
}

\chadded{
Given that a type checker can identify a broad range of issues beyond variable misuse, we adopt the filtering approach similar to that described in \autoref{fig:bug-label}, focusing exclusively on the subset of type-related bugs appeared in the distribution observed for variable misuse errors (\autoref{fig:error-type}). This approach resulted in the type checker achieving a \textbf{CPR} of 98.46\%. \autoref{tab:pipeline} shows the performance of the bug detection pipeline in \autoref{fig:motivation}. The pipeline provides a notable improvement to bug localization while marginally reducing correct program recall. We suspect that the reduction in correct program recall is due to the type checker and the neural bug detectors tending to raise false alarms on different programs.
}

\begin{tcolorbox}
\textbf{RQ2}: 
Our findings reveal that bug detectors exhibit superior performance in detecting type-related bugs compared to other types of bugs. The removal of these bugs from the evaluation dataset leads to a reduction in bug localization accuracy by up to 5.61\%. This suggests that the inclusion of type-related bugs in the evaluation dataset, particularly when utilizing a type checker, may yield overly optimistic evaluation results.

% Irrespective of the training paradigm or model architecture, our observations indicate that neural bug detectors consistently exhibit better performance on type-related bugs compared to other bugs. Additionally, despite type-related bugs constituting less than $20\%$ of the dataset, their removal results in a reduction of up to $5.61\%$ in the detector's bug localization accuracy. This suggests that type-related bugs are relatively easier to identify for neural bug detectors trained on synthetic datasets. Consequently, the presence of type-related bugs in the evaluation dataset may lead to overly optimistic evaluation results.

\end{tcolorbox}


\subsection{RQ3: Effect of type-related bugs on training}

\subsubsection{Addressing the RQ}
In this section, we investigate the impact of filtering type-related bugs from the training data on the performance of the neural bug detectors. Neural bug detectors trained with the \emph{full dataset} are compared with those trained with the \emph{filtered dataset} using both correct program recall and location accuracy on all samples from the evaluation datasets.

%\textbf{Training Dataset Preparation}
A naive approach to filter type-related bugs from the training data is to remove all samples that are identified as type-related bugs. However, this approach may result in a significant reduction in the size of the training data as well as an imbalance in the correct and faulty programs. To mitigate these issues, we \textit{replace} the type-related bugs with other bugs in the training data by randomly oversampling other bugs in the dataset. This approach ensures that the size of the training data remains the same and the balance between correct and faulty programs is maintained.

%\textbf{Evaluation}
\todo[inline]{move the paragraph "We target..." to the 2nd in this section}We target to measure the practical performance of neural bug detectors in a real-world setting where a type checker is integrated in the development process. Thus, we only focus on bugs that are beyond the scope of type checkers and filter all type-related bugs from the evaluation datasets. 

\subsubsection{Results}

The performance change of neural bug detectors trained with full dataset and filtered dataset is shown in \autoref{tab:impact-training}. Values on the left side of the arrow show the performance of the full training dataset while the right side represents the performance of filtered training. The numbers after the dashed line show the relative change in performance of the two versions of training datasets. Correct program recall for \emph{Real-PyPI} is not available as the dataset only contains faulty programs.

In general, the localization accuracy experiences enhancement when the neural bug detector is trained on the filtered dataset, as observed in 13 out of 15 cases. This enhancement is particularly prominent in real-world datasets, with average increases of $3.52\%$ and $5.73\%$ for Real-Py150 and Real-PyPI, respectively. This improvement can be attributed to the elimination of type-related bugs from the training data, enabling the neural bug detectors to concentrate more on detecting other types of bugs beyond the limitations of a type checker.

%The improvement can be as high as 10.11\% for the GraphCodeBert in the \emph{Real-PyPI} dataset. Such improvement can be explained by the removal of type-related bugs from the training data, which allows the neural bug detectors to focus more on other types of bugs beyond the scope of a type checker. Moreover, the performance gain is generally more significant in the real world datasets compared to the synthetic datasets. This improvement means that the filtering dataset is generally more effective in practical settings.

Additionally, we also note a decrease in correct program recall in 8 out of 10 cases. However, this reduction is considerably less notable compared to the enhancement in localization accuracy. Specifically,  the average change ratio for \textbf{LA} is about $2.44\times$ the average change ratio for \textbf{CPR} in the synthetic datasets and $13.04\times$ in the \textit{Real-Py150} dataset. We hypothesize that this phenomenon may be attributed to the oversampling strategy we employed, rather than generating entirely new synthetic samples.

%Nevertheless, a decrease in the correct program recall is also observed for a significant number of cases (8/10), though the decrease is generally less significant compared to the improvement in the localization accuracy. 

%The highest decrease is observed in the \emph{Real-Py150} dataset, where the correct program recall decreases by 0.57\% for UnixCoder. We suspect such a decrease is not statistically significant and is likely due to the random sampling during the replacement of type-related bugs in the training data.

%\chadded{
%Comparing the impact of training on the filtered dataset on \textbf{CPR} and \textbf{LA}, we observe that the impact on \textbf{LA} is much more significant than the impact on \textbf{CPR}. The average change ratio for \textbf{LA} is about $2.44\times$ the average change ratio for \textbf{CPR} in the synthetic datasets and $13.04\times$ in the \textit{Real-Py150} dataset. Such observation confirms that the removal of type-related bugs from the training data generally provides more improvement than the decrease in correct program recall.
%}

% To measure the statistic significance of the performance change, we perform Wilcoxon signed-rank test on the performance change of the neural bug detectors. When checking the significance of the performance change in \textbf{CPR} with alternative hypothesis that the mean of performance change is less than zero, a p-value of 0.14 is obtained, indicating that the performance change is not statistically significant. However, when checking the significance in \textbf{LA} with alternative hypothesis that the mean of performance change is greater than zero, a p-value of 0.003 is obtained, indicating that the performance change is statistically significant.

% Furthermore, we also calculate the effect size pf the Wilcoxon signed-rank test of the performance change for each dataset, which is shown in the last row of \autoref{tab:impact-training}. The effect size is calculated using the formula $r = Z/\sqrt{N}$, where $Z$ is the z-score of the test and $N$ is the number of samples. Similarly, we observe that the effect size of the performance change in \textbf{LA} is generally larger than the effect size of the performance change in \textbf{CPR}, indicating that the performance change in \textbf{LA} is more significant.


 
% \todo{Size effect for each column}
\begin{table*}[tb]
    \centering
    \caption{Performance change of detectors trained with full dataset and filtered dataset. Numbers are in percentage. Numbers after the dashed line show the relative change in performance. In general, filtering type-related bugs in training improves the localization accuracy but decreases the correct program recall.}
    \begin{tabular}{|c|c:cc:c|c:cc:c|cc:c|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{Synthetic} & \multicolumn{4}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
    \cline{2-12}
    & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR}& \textbf{LA} & $\Delta$\\
    \hline
    CodeBert      & 95.94 $\rightarrow$ 95.54 & -0.42 & 92.90 $\rightarrow$ 93.23 & 0.36 & 95.61 $\rightarrow$ 95.31 & -0.32 & 35.33 $\rightarrow$ 35.43 &  0.27 & -- & 33.42 $\rightarrow$ 32.35 & -3.20 \\
    GraphCodeBert & 96.27 $\rightarrow$ 95.90 & -0.38 & 93.82 $\rightarrow$ 94.01 & 0.20 & 96.09 $\rightarrow$ 95.63 & -0.48 & 36.50 $\rightarrow$ 39.21 &  7.43 & -- & 33.29 $\rightarrow$ 36.63 &  10.04 \\
    UnixCoder     & 96.23 $\rightarrow$ 95.83 & -0.42 & 93.70 $\rightarrow$ 93.98 & 0.30 & 96.05 $\rightarrow$ 95.51 & -0.57 & 36.27 $\rightarrow$ 38.48 &  6.08 & -- & 33.29 $\rightarrow$ 35.89 &  7.81 \\
    GGNN          & 92.97 $\rightarrow$ 92.74 & -0.25 & 72.64 $\rightarrow$ 73.30 & 0.91 & 92.64 $\rightarrow$ 92.16 & -0.51 & 14.76 $\rightarrow$ 14.67 & -0.63 & -- & 15.18 $\rightarrow$ 15.76 &  3.88 \\
    GREAT         & 90.56 $\rightarrow$ 91.07 &  0.56 & 81.51 $\rightarrow$ 81.88 & 0.45 & 88.96 $\rightarrow$ 89.43 &  0.52 & 20.89 $\rightarrow$ 21.82 &  4.44 & -- & 20.94 $\rightarrow$ 23.06 &  10.11 \\
    \hhline{============}
    Average & \multicolumn{2}{r}{-0.18} & \multicolumn{2}{r|}{0.44} & \multicolumn{2}{r}{-0.27} & \multicolumn{2}{r|}{3.52} & -- & \multicolumn{2}{r|}{5.73}\\
    \hline
    \end{tabular}
    
    \label{tab:impact-training} 
\end{table*}

% \begin{table*}[tb]
%     \centering
%     \caption{Performance change of model trained with dataset excluding type-related bugs compared to the full synthetic dataset. A positive value means an improvement from the training with the full dataset}
%     \begin{tabular}{|c|c|c|c||c|c|c||c|c|c|}
%     \hline
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c||}{Synthetic 1} & \multicolumn{3}{c||}{Synthetic 2} & \multicolumn{3}{c|}{Real} \\
%     \cline{2-10}
%     & \textbf{CPR} & \textbf{LA} & \textbf{Joint} & \textbf{CPR} & \textbf{LA} & \textbf{Joint} & \textbf{CPR} & \textbf{LA} & \textbf{Joint}\\
%     \hline
%     CodeBert & -0.45 &  0.38 & -0.10 & -0.04 &  0.05 &  0.00 & -0.31 &  0.10 & -0.29 \\
%     GraphCodeBert & -0.47 &  0.39 & -0.10 &  0.06 &  0.43 &  0.22 & -0.46 &  2.71 & -0.37 \\
%     UnixCoder & -0.32 &  0.32 & -0.04 & -0.31 &  0.62 &  0.11 & -0.55 &  2.20 & -0.46 \\
%     GGNN & -0.28 &  0.62 &  0.13 & -0.49 & -1.83 & -1.15 & -0.29 &  0.18 & -0.27 \\
%     GREAT &  0.71 &  0.27 &  0.51 &  0.36 & -1.64 & -0.63 & 0.43 &  1.39 &  0.48 \\
%     Transformer & -3.88 & -1.99 & -3.03 & -3.37 & -2.43 & -2.91 & -2.76 & -1.20 & -2.68 \\
%     \hline
%     \end{tabular}
    
%     \label{tab:type oversampling} 
% \end{table*}

% \todo{Add rq headers to other parts}
\begin{tcolorbox}
    \textbf{RQ3}: Removing type-related errors from the training dataset causes a significant increase in localization accuracy. Although a decrease in correct program recall is also noted, it is substantially less significant.
    
    %In general, we observe that the performance of neural bug detectors trained without type-related bugs has a better localization accuracy (in 13/15 cases) while reducing the correct program recall (in 8/10 cases). This finding indicates that while type-related bugs diminish the detector's ability to localize bugs, they contribute positively to the detector's ability to decide if a program contains an error.
\end{tcolorbox}

==> initial-version/sections/evaluation_new.tex <==
\section{Effect of Type Checking}
\label{sec:effect}

\subsection{Motivation}


%Though type-related errors exist in both synthetic and real-world datasets, the former contains a much higher proportion of such bugs. 
Neural bug detection datasets contain a significant proportion of type-related bugs, indicating the potential application of type checkers in detecting these bugs. In this section, we investigate how and when a type checker should be used together with a neural bug detector for dynamically typed languages. Moreover, in scenarios where a type checker is used, neural bug detectors are expected not to analyze bugs detectable by the type checker. Thus, to offer recommendations for deploying neural bug detectors alongside a type checker, it is crucial to understand the impact of type-related bugs on the training and testing of these neural systems. As a result, we aim to address the following three research questions:


%In real world setting when a type checker is deployed in development, the type-related bugs are often caught before by the type checker 

%they are pushed into the code base by a type checker. Thus, it is important to understand how type-related errors influence the training and testing of the the neural bug detectors. Specifically, we investigate the following two research questions:

%This section presents our experiment results demonstrating the effect of type-related bugs on the performance of these neural bug detectors in both evaluation and training. Specifically, we investigate the following two research questions:

\begin{itemize}
    \item \textbf{RQ2:} How does type checking influence the performance of neural bug detection when they are used together?
    \item \textbf{RQ3:} How do type-related bugs influence the evaluation of neural bug detectors?
    \item \textbf{RQ4:} How do type-related bugs influence the training of neural bug detectors?
\end{itemize}


\subsection{Experiment setup}
We introduce the neural networks used in the neural bug detectors in our experiments. This is followed by datasets and evaluation metrics used to investigate the research questions. 


\begin{table}[tb]
    \centering
    \caption{Bug Detection Neural Networks used in the experiments}
    \begin{tabular}{cccc}
    \hline
    \textsc{Model} & \textsc{Architecture} & \textsc{Training strategy} \\
    \hline
    GGNN \cite{allamanis2017learning} & GNN & From scratch \\
    % \hline
    % 6-layer transformer \cite{hellendoorn2019global} & Transformer & Full \\

    CodeBERT \cite{feng2020codebert} & Transformer & Fine-tuning \\

    GraphCodeBERT \cite{guo2020graphcodebert} & Transformer & Fine-tuning \\

    UnixCoder \cite{guo2022unixcoder} & Transformer & Fine-tuning \\

    GREAT \cite{hellendoorn2019global} & Hybrid & From scratch \\
    \hline
    \end{tabular}
    \label{tab:models}
\end{table}

\subsubsection{Neural bug detectors}


The first column of \autoref{tab:models} shows the neural bug detectors used in our experiments. The second column illustrates the architectures corresponding to each considered model. We cover three widely employed architectures: transformers, GNNs, and hybrid methods. Lastly, the third column denotes whether the detector is trained from scratch (\textit{i.e.,} initialized with random weights) or fine-tuned (\textit{i.e.,} initialized with a pre-trained neural network).

%In this paper, we focus on three main architectures of neural networks: graph neural networks, transformers, and hybrid methods. Furthermore, they can also be categorized by the training strategy: full training or fine-tuning. \autoref{tab:models} presents the neural networks used in our experiments.

%When fine-tuning a pre-trained model, we follow previous work \cite{troshin2022probing} by appending a classification layer to the pre-trained model and fine-tuning the entire model. For the full training models, we adapt the implementation from previous work \cite{hellendoorn2019global}

\subsubsection{Datasets}
We adopt the methodology established in prior studies concerning training with a synthetic dataset and assessed using both the synthetic test split from the same dataset and real-world datasets~\cite{hellendoorn2019global,habib2019neural,he2022distribution,richter2023train}. Specifically, we select the \synthetic{} dataset as our training dataset because of its larger volume of data.
%For detecting variable misuse task, we use the training split of the \textit{Synthetic 1} due to its larger amount of data and its distribution of type-related errors is closely aligned with that of real-world scenarios. Subsequently, we evaluate the trained models also on the test split of the dataset.

The trained neural bug detectors are also evaluated on both real-world datasets: \realpy{} and \realpypi{}. All processed variable misuse bugs from the \realpypi{} dataset are also included in the evaluation. Then, the two datasets are merged together as the \real{} evaluation dataset to cover both correct programs as well as a diverse set of faulty programs.

%\textbf{Data leakage check}
Since the real-world datasets are constructed independently from the \synthetic{} dataset, some of the real-world bug programs may also appear in the training set of \synthetic{}. To avoid such data leakage issues, all potential duplicated samples are excluded from the real-world datasets during evaluation. Specifically, we use the metadata of each sample as a heuristic and remove all program samples that are from the same file in the same repository and have the same function signature as any samples from the synthetic training set. In total, 42.62\% correct programs and 7.89\% of bugs in the \realpy{} dataset, and 0.48\% of faulty programs in the \realpypi{} dataset are removed due to potential duplication with the training data. 

% We suspect the high duplication rate in \realpy{} is due to its construction using the same repositories as \synthetic{}.

% We perform data leakage check on the \textit{VarMisuseReal} dataset and found it does not contain any files from the repositories as the synthetic dataset. Thus, we include all faulty programs from this dataset and randomly sample the same number of correct programs to build a balanced real world test set.

\subsubsection{Metrics}
In this work, we evaluate the performance of neural bug detectors as a classification problem. Compared to standard classification metrics, we define stricter true positive cases for a bug detection task, taking into account bug localization. Specifically, given a set of faulty programs $\mathcal{P}_f$ and a bug detector $\mathfrak{D}$, the true positives ($TP$) are defined as the number of programs where the bug detector correctly identifies \emph{and} localizes the bug:
$$    TP(\mathfrak{D}, \mathcal{P}_f) = |\{p\in\mathcal{P}_f|d_{\mathfrak{D}(p)} = \texttt{true} \land l_{\mathfrak{D}(p)} = l_p\}|$$
where $d_{\mathfrak{D}(p)}$ represent decision and $l_{\mathfrak{D}(p)}$ represent the bug location of the program $p$ predicted by the neural bug detector. Then, all other programs $p$ with $d_{\mathfrak{D}(p)} = \texttt{true}$ are considered as \emph{false positives} ($FP$). 
Moreover, false negatives ($FN$) are the number of faulty programs where the bug detector wrongly identifies the program as bug-free. Formally, the false negative ($FN$) is defined as the following:
$$    FN(\mathfrak{D}, \mathcal{P}_f) = |\{p\in\mathcal{P}_f|d_{\mathfrak{D}(p)} = \texttt{false}\}|$$

Finally, all other programs the neural bug detector identifies as bug-free are considered as \emph{true negative} ($TN$). 

To evaluate the performance with neural bug detectors, we use standard precision and recall as metrics:
$$    \text{Precision} = \frac{TP}{TP + FP}\:\:\:\:\text{Recall} = \frac{TP}{TP + FN}$$
To evaluate the joint performance of the bug detector, the F-score is typically used. However, the F-1 score treats precision and recall equally. In a real-world scenario, a programmer may prefer a higher recall to ensure all bugs are detected, even if it means more false positives, or a higher precision to reduce the number of false alarms. Therefore, we consider the \fbeta{} score~\cite{goutte2005probabilistic}, which allows us to adjust the importance of precision and recall. Specifically, the \fbeta{} score is defined as:
$$
    F_{\beta} = (1 + \beta^2) \times \frac{\text{Precision} \times \text{Recall}}{\beta^2 \times \text{Precision} + \text{Recall}}$$
while $\beta$ represents the relative importance of recall compared to precision. A higher $\beta$ signifies more emphasis on recall. When $\beta = 1$, the \fbeta{} score is equivalent to the F-1 score. In a software engineering context, a higher $\beta$ is preferable when detecting and fixing bugs are costly and time-consuming, while a lower $\beta$ is appropriate when developers need to spend much time on checking false alarms of automated detection tools.
%\todo[inline]{Check the practical implication}

To measure the differences in performance of the two settings, we use \emph{ratio change}. Given the performance values of two settings $p_a$ and $p_b$, the ratio change $\Delta$ of $p_b$ with respect to $p_a$ is calculated as follows:
\begin{equation*}
    \Delta = \frac{p_b - p_a}{p_a} \times 100
\end{equation*}

\noindent\textbf{Comparison to existing metrics.}
Existing work often uses correct program recall and localization accuracy as the metrics for a neural bug detector \cite{hellendoorn2019global,habib2019neural} to evaluate bug classification and localization separately. In fact, the definition of localization accuracy is the same as recall in our metrics. While the correct program recall is equivalent to the true negative rate in our setting. Furthermore, the \fbeta{} score takes both metrics into account and can provide a more comprehensive evaluation of the neural bug detectors' end-to-end performance.

% Following previous work \cite{hellendoorn2019global,habib2019neural}, we use separate metrics for bug classification and localization. First, we measure the \textit{correct program recall} (\textbf{CPR}), which is the recall of a neural bug detector in deciding that a program is free from any bugs. Specifically, given a neural bug detector and a set of \emph{correct} programs $\mathcal{P}_c$, the \textbf{CPR} is defined as:
% \begin{equation*}
%     CPR(\mathfrak{D}, \mathcal{P}_c) = \frac{|\{p\in\mathcal{P}_c|d_{\mathfrak{D}(p)} = \texttt{false}\}|}{|\mathcal{P}_c|}
% \end{equation*}
% where $d_{\mathfrak{D}(p)}$ represents the decision of the neural bug detector on the program.

% Then, for all the faulty programs, we measure the \textit{location accuracy} (\textbf{LA}) which is the proportion of programs where the model correctly identifies the location of the bug. Let $\mathcal{P}_f$ represent the set of \emph{faulty} programs and $l_p$ represent the location of the bug for the program $p$, \textbf{LA} is defined as follows.
% \begin{equation*}
%     LA(\mathfrak{D}, \mathcal{P}_f) = \frac{|\{p\in\mathcal{P}_f|d_{\mathfrak{D}(p)} = \texttt{true} \land l_{\mathfrak{D}(p)} = l_p\}|}{|\mathcal{P}_f|}
% \end{equation*}
% where $l_{\mathfrak{D}(p)}$ represent the bug location of the faulty program $p$ predicted by the neural bug detector.

% \chadded{
% Finally, to measure the differences in performance of the two settings, we use \emph{ratio change}. Given the performance values of two settings $p_a$ and $p_b$, the ratio change $\Delta$ of $p_b$ with respect to $p_a$ is calculated as follows:
% }
% \begin{equation*}
%     \Delta = \frac{p_b - p_a}{p_a} \times 100
% \end{equation*}

\subsubsection{Training settings}
Previous work often trains the neural bug detector with the joint training objective of both bug detection and repair \cite{VasicKMBS19,allamanis2017learning,hellendoorn2019global}. In our preliminary experimentation, we notice that training without the repairing loss results in either similar or degraded performance compared to the joint objective. Consequently, we opt to use the joint training objective, as done in previous studies.

When training GGNN and GREAT models, we use the same hyperparameter configurations as in previous work~\cite{hellendoorn2019global} and train for 5 and 10 epochs, respectively. For fine-tuning, we train each model for 1 epoch and use a learning rate of $1^{-5}$ with a linear learning rate scheduler.

\subsection{RQ2: Influence of type checker}
\label{sec:influence-type-check}
\subsubsection{Addressing the RQ}
In this section, we aim to (A) evaluate the effect of integrating a type checker into the neural bug detector similar to the ones used for statically typed languages as shown in \autoref{fig:motivation} and (B) investigate when and how the type checker should be used together with the neural bug detector depending on the requirement of the developer. 

All neural bug detectors are trained with the synthetic dataset on the variable misuse task. To gain insights on the influence of type checkers in a practical scenario, we evaluate the performance of the bug detectors on the \emph{Real} dataset. In general, for each neural bug detector, we consider two settings: 1) \textbf{NN}: the neural bug detector is used alone and 2) \textbf{Pipeline}: the neural bug detector is used together with a type checker in a pipeline as shown in \autoref{fig:motivation}. 

We also evaluate the precision and recall of the type checker using the \textit{Real} dataset. Specifically, we define $TP$ as the count of buggy samples correctly identified by the type checker (i.e., bugs listed in \autoref{tab:existance}). $FN$ represents buggy samples missed by the type checker. Additionally, we determine $FP$ by running the type checker on the correct programs. A correct program is classified as $FP$ if the type checker raises an error categorized under variable misuse errors (\autoref{fig:error-type}). This criterion is adopted because the type checker's capability extends to detecting various bug types beyond variable misuse.

%We use the proportion of type-related bugs identified by the type checker in \autoref{tab:existance} as the positive samples for the type checker. Then, type checking is also performed for all correct programs in the dataset to identify potential false positives. Since a type checker can identify a broad range of bugs beyond variable misuse, we adopt the filtering approach similar to that described in \autoref{fig:bug-label}, focusing exclusively on the subset of type-related bugs that appeared in the distribution observed for variable misuse errors (\autoref{fig:error-type}).
% This approach resulted in the type checker achieving a CPR of 98.46%.

\subsubsection{Results}
\begin{table}[tb]
    \centering
    \caption{Precision and recall of the bug detectors on the Real dataset. Numbers are in percentage. The pipeline setting always improves recall but may reduce precision.}
    \begin{tabular}{|c|cc|cc|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{Precision} & \multicolumn{2}{c|}{Recall} \\
    \cline{2-5}
    & \textbf{NN} & \textbf{Pipeline} & \textbf{NN} & \textbf{Pipeline}\\
    \hline
    CodeBert      & \textbf{28.00} & 25.23 & 32.26 & \textbf{35.58}\\
    GraphCodeBert & \textbf{30.84} & 27.13 & 32.59 & \textbf{35.81}\\
    UnixCoder     & \textbf{31.85} & 27.98 & 34.56 & \textbf{37.69}\\
    GGNN          & 10.51 & \textbf{11.31} & 17.29 & \textbf{21.81}\\
    GREAT         &  9.92 & \textbf{10.35} & 26.69 & \textbf{30.49}\\
    \hline
    \texttt{pytype} & \multicolumn{2}{c|}{17.83} & \multicolumn{2}{c|}{5.01} \\
    \hline
    \end{tabular}
    
    \label{tab:pipeline-precision-recall}
\end{table}

\autoref{tab:pipeline-precision-recall} shows the precision and recall of the neural bug detectors in the \textit{Real} dataset for both the \textbf{NN} and \textbf{Pipeline} settings, and results of the type checker (\texttt{pytype}). 

% Although the type checker generally produces fewer false positives than neural bug detectors, its precision remains low at 17.83 due to the small number of type-related bugs identified compared to the neural bug detectors. Furthermore, we adopt the same configuration for all programs in the dataset. In practice, one can adjust the type checker's configuration based on the project, potentially leading to improved performance.

The type checker exhibits reasonable precision but low recall in identifying variable misuse bugs. This limited performance may be attributed to using a single type checker configuration for all programs in the dataset. In practice, one can adjust the type checker's configuration based on the project to further reduce false alarms.

%The type checker exhibits low precision in identifying variable misuse bugs. We suspect this is because a single type checking configuration is used for all programs in the dataset. In practice, one can adjust the type checker's configuration based on the project to further reduce false alarms.

%Although the precision and recall of the type checker are low, the 
Neural bug detectors in the \textbf{Pipeline} configuration demonstrate higher recall than those in the \textbf{NN} setup. Additionally, for certain models (GGNN and GREAT), the precision also improves. 
This is likely caused by the fact that the type checker has better precision than these neural bug detectors.

The recall improvement ranges from 3.13\% to 4.51\% for all neural bug detectors, indicating that integrating a type checker into the bug detection can help identify more bugs. However, the precision of the neural bug detectors in the \textbf{Pipeline} setting also decreases for all pre-trained models due to the new false positives introduced by the type checker.

% This reduction in precision is rooted from the fact that integrating a type checker may also lead to more false alarms as the type checker may catch bugs other than variable misuse. 


\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{imgs/fbeta_score}
    \caption{\fbeta{} score for different values of $\beta$ of the neural bug detectors in the \textbf{NN} (solid) and \textbf{Pipeline} (dashed) settings. The \textbf{Pipeline} setting surpasses the \textbf{NN} setting for all neural bug detectors when $\beta\geq1.34$.}
    \label{fig:f-beta}
\end{figure}

To better understand the trade-off between precision and recall introduced by the type checker, we plot the \fbeta{} score for different values of $\beta$ in \autoref{fig:f-beta}. The two full training methods are excluded as the \pipeline{} approach improves both precision and recall. In general, when $\beta=1$, the \nn{} setting achieves a higher score compared to the \pipeline{} setting, indicating that it may not be necessary to include type checking when the frequency of false alarms is a concern. However, when $\beta \ge 1.34$ (\textit{i.e.,} recall is considered $1.34$ times more important than precision), the \pipeline{} setting surpasses the \nn{} setting for all neural bug detectors, suggesting that the type checker can be beneficial when revealing bugs in the code is a priority.

For the rest of the paper, we consider both $\beta=1$ and $\beta=1.5$, for cases where precision and recall hold equal importance and scenarios where bug identification is more critical.

% Since a type checker is more valuable when recall of bugs is more important, its combination with the neural bug detectors is likely in such scenarios. For the rest of the paper, we take both $\beta=1$ and $\beta=1.5$ to consider 

% Thus, for the rest of the paper, we fix $\beta=1.5$ to evaluate the performance of the neural bug detectors under the \pipeline{} setting.


\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
    \textbf{RQ2}: Combining a type checker with neural bug detectors can improve recall up to 4.51\%, but it may reduce precision up to 3.86\%. The trade-off between precision and recall depends on the relative importance of identifying bugs and reducing false alarms. When identifying bugs is more important, a type checker should be used.
\end{tcolorbox}
    


\subsection{RQ3: Evaluation on type-related bugs}
\subsubsection{Addressing the RQ}
Since integrating type checkers can be beneficial if identifying bugs is key, when using a type checker in combination with a neural bug detector, the neural bug detector should mainly focus on the bugs that are not easily detectable by the type checker. In this section, we evaluate the performance of neural bug detectors on type-related bugs compared to other bugs when trained with a synthetic dataset on the variable misuse task. We divide the evaluation dataset into two groups based on the type-checking results in the evaluation: type-related bugs and other bugs. 
%We then evaluate the recall of the neural networks on these two groups of bugs separately.
We then show the impact of the type-related bugs on the overall performance by evaluating programs and programs filtering type-related bugs. In this experiment, we consider both \synthetic{} and \real{} datasets.

\begin{table*}[tb]
    \centering
    \caption{Impact of filtering type-related bugs on precision and recall Numbers are in percentage. \\Removing type-related bugs reduces the performance of neural bug detectors in both precision and recall. }
 
    \begin{tabular}{|c|ccc|ccc||ccc|ccc|}
    \hline
    \multirow{3}{*}{\textbf{Model}} &\multicolumn{6}{c||}{\synthetic{}} & \multicolumn{6}{c|}{\real{}}\\
    \cline{2-13}
    & \multicolumn{3}{c|}{Precision} & \multicolumn{3}{c||}{Recall} & \multicolumn{3}{c|}{Precision} & \multicolumn{3}{c|}{Recall} \\
    \cline{2-13}
    & \textbf{Full} & \textbf{Filtered} & $\Delta$ & \textbf{Full} & \textbf{Filtered} & $\Delta$ & \textbf{Full} & \textbf{Filtered} &$\Delta$ & \textbf{Full} & \textbf{Filtered} &$\Delta$\\
    \hline
    CodeBert      & 93.40 & 91.91 & -1.59 & 91.67 & 90.77 & -0.98 & 28.00 & 26.96 & -3.70 &   32.26 & 31.85 & -1.29\\
    GraphCodeBert & 94.00 & 92.63 & -1.46 & 92.19 & 91.38 & -0.88 & 30.84 & 29.63 & -3.94 &   32.59 & 32.12 & -1.43\\
    UnixCoder     & 94.07 & 92.70 & -1.45 & 93.58 & 92.79 & -0.84 & 31.85 & 30.68 & -3.65 &   34.56 & 34.10 & -1.31\\
    GGNN          & 86.38 & 83.12 & -3.77 & 80.89 & 77.31 & -4.42 & 10.51 & 9.82 & -6.56 & 17.29 & 16.86 & -2.50\\
    GREAT         & 84.80 & 81.44 & -3.97 & 89.68 & 87.53 & -2.39 & 9.92 & 9.17 & -7.60 & 26.69 & 25.70 & -3.71\\
    \hline
    \end{tabular}    
    \label{tab:type-impact}
\end{table*}

\subsubsection{Results}
\autoref{tab:type-impact} shows the precision, and recall before and after filtering type-related bugs from the evaluation datasets. The \fbeta{} score is excluded from the table as both precision and recall decrease for all settings.

Comparing the performance of the neural bug detectors on synthetic and real-world datasets, we observe that these detectors perform much better on the synthetic datasets compared to the real-world bugs, consistent with previous work~\cite{he2022distribution,allamanis2021self}. This discrepancy can be attributed to the distribution shift between synthetic and real-world bugs~\cite{he2022distribution}. 

% Neural bug detectors consistently perform better in identifying type-related bugs, with a difference reaching up to 34.71\% for GraphCodeBert within the \emph{Real-PyPI} dataset. This finding aligns with our observations from the previous research question regarding the trivial nature of type-related bugs.

%indicates that neural bug detectors are indeed better at identifying type-related bugs with are composed of a large portion of trivial errors as shown in \autoref{fig:error-type} 


To evaluate the impact of type-related bugs on precision and recall, we include the ratio of change in the filtered dataset compared to the full dataset, denoted as $\Delta$ in the table. We observe a decrease in both precision and recall for all neural bug detectors in the filtered evaluation set, suggesting a bias of neural bug detectors towards type-related bugs. The most significant decrease in precision is noted in the \real{} dataset, with a reduction of 7.60\% for the GREAT model. The highest reduction in recall of 4.42\% is observed for GGNN in \synthetic{}. This finding implies that the presence of type-related bugs in the evaluation dataset may lead to overly optimistic evaluation outcomes, especially when a type checker is used in the pipeline.

Furthermore, the decline in performance is notably more significant for the real-world dataset compared to the synthetic dataset. This observation brings increased threats to evaluation validity in real-world use cases compared to synthetic datasets.

% Since all neural bug detectors perform better on type-related bugs, we observe that the removal of type-related bugs generally reduces the performance of the neural bug detectors. The highest reduction is observed in the \emph{Real-PyPI} dataset, where the removal of type-related bugs results in a reduction of up to 5.61\% for the GREAT model, even though the type-related bugs only constitute 4\% of the dataset.

%In general, models using a full training strategy tends to bias more towards type-related bugs compared to fine-tuning models. This can be explained by fine-tuning models are already pre-trained with a large amount of code data and thus are less likely to be influenced by the type-related bugs in the training data. At the same time, the impact of type-related bugs on the performance also varies across different datasets, with the highest impact observed in the \emph{Real-PyPI} dataset and the lowest in the \emph{Real-Py150} dataset.

% \chadded{
% Our observations indicate that, despite being comparatively more effective than other bug types, the performance of neural bug detectors for identifying type-related bugs in real-world datasets remains suboptimal. Therefore, integrating neural bug detectors with a type checker within the pipeline as depicted in \autoref{fig:motivation}, is expected to enhance the performance in bug localization. To evaluate the performance of this integrated pipeline, we conducted experiments using the type checker on the correct programs within the \emph{Real-Py150} dataset. 
% }

% \chadded{
% Given that a type checker can identify a broad range of issues beyond variable misuse, we adopt the filtering approach similar to that described in \autoref{fig:bug-label}, focusing exclusively on the subset of type-related bugs appeared in the distribution observed for variable misuse errors (\autoref{fig:error-type}). This approach resulted in the type checker achieving a \textbf{CPR} of 98.46\%. \autoref{tab:pipeline} shows the performance of the bug detection pipeline in \autoref{fig:motivation}. The pipeline provides a notable improvement to bug localization while marginally reducing correct program recall. We suspect that the reduction in correct program recall is due to the type checker and the neural bug detectors tending to raise false alarms on different programs.
% }

\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
\textbf{RQ3}: 
Our findings reveal that bug detectors exhibit superior performance in detecting type-related bugs compared to other types of bugs. Removing these bugs from the evaluation dataset leads to a reduction in both precision (up to 7.60\%) and recall (up to 4.42\%). This suggests that the inclusion of type-related bugs in the evaluation dataset, particularly when using a type checker, may yield overly optimistic evaluation results.

\end{tcolorbox}


\subsection{RQ4: Effect of type-related bugs on training}

\subsubsection{Addressing the RQ}
In this section, we investigate the impact of filtering type-related bugs from the training data on the performance of the neural bug detectors. Neural bug detectors trained with the \emph{full dataset} are compared with those trained with the \emph{filtered dataset} using precision, recall, and \fbeta{} on all samples from the evaluation datasets, excluding type-related bugs. We aim to measure the performance of neural bug detectors when the type checker is used together as a pipeline. Thus, we only focus on bugs beyond the scope of type checkers and filter all type-related bugs from the datasets. 

%\textbf{Training Dataset Preparation}
A naive approach to filter type-related bugs from the training data is to remove all samples identified as type-related bugs. However, this approach may result in a significant reduction in the size of the training data as well as in an imbalance in the correct and faulty programs. To mitigate these issues, we \textit{replace} the type-related bugs with other bugs in the training data by randomly oversampling other bugs. This approach ensures that the size of the training data remains the same and the balance between correct and faulty programs is maintained.

%\textbf{Evaluation}
% \todo[inline]{move the paragraph "We target..." to the 2nd in this section}

\begin{table*}[tb]
    \centering
    \caption{Performance of detectors trained with full dataset $\rightarrow$ filtered dataset. Numbers are in percentage.\\ In general, filtering type-related bugs in training improves the recall while decreasing the precision.}
    \begin{tabular}{|c|cccc|cccc|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\synthetic{}} & \multicolumn{4}{c|}{\textit{Real}} \\
    \cline{2-9}
    & \textbf{Precision} & \textbf{Recall} & F-1 & \fbeta{} ($\beta=1.5$) & \textbf{Precision} & \textbf{Recall} & F-1 & \fbeta{} ($\beta=1.5$)\\
    \hline
    CodeBert      & 91.91$\rightarrow$91.38 &  90.77$\rightarrow$91.17 & \textbf{91.33}$\rightarrow$91.28 & 91.12$\rightarrow$\textbf{91.23} &  26.96$\rightarrow$25.48 &  31.85$\rightarrow$31.67 & \textbf{29.20}$\rightarrow$28.24 & \textbf{30.17}$\rightarrow$29.47 \\
    GraphCodeBert & 92.63$\rightarrow$92.12 &  91.38$\rightarrow$91.65 & \textbf{92.00}$\rightarrow$91.88 & 91.76$\rightarrow$\textbf{91.79} &  29.63$\rightarrow$29.25 &  32.12$\rightarrow$34.87 & 30.82$\rightarrow$\textbf{31.82} & 31.31$\rightarrow$\textbf{32.93} \\
    UnixCoder     & 92.70$\rightarrow$92.22 &  92.79$\rightarrow$93.10 & \textbf{92.75}$\rightarrow$92.66 & 92.76$\rightarrow$\textbf{92.83} &  30.68$\rightarrow$29.49 &  34.10$\rightarrow$36.60 & 32.30$\rightarrow$\textbf{32.67} & 32.97$\rightarrow$\textbf{34.08} \\
    GGNN          & 83.12$\rightarrow$82.78 &  77.31$\rightarrow$78.18 & 80.11$\rightarrow$\textbf{80.42} & 79.01$\rightarrow$\textbf{79.54} &   9.82$\rightarrow$9.42  &  16.86$\rightarrow$17.17 & \textbf{12.41}$\rightarrow$12.17 & \textbf{13.82}$\rightarrow$13.70 \\
    GREAT         & 81.44$\rightarrow$82.20 &  87.53$\rightarrow$87.72 & 84.38$\rightarrow$\textbf{84.87} & 85.56$\rightarrow$\textbf{85.95} &   9.17$\rightarrow$10.13 &  25.70$\rightarrow$27.19 & 13.51$\rightarrow$\textbf{14.76} & 16.53$\rightarrow$\textbf{17.91} \\
    \hline
    \end{tabular}
    
    \label{tab:impact-training} 
\end{table*}


\subsubsection{Results}

The performance change of neural bug detectors trained with the full dataset and the filtered dataset is shown in \autoref{tab:impact-training}. Values on the left side of the arrow show the performance of the full training dataset while the right side represents the performance of filtered training. The better \fbeta{} scores of the two settings are highlighted in bold.

%The numbers after the dashed line show the relative change in performance of the two versions of training datasets. Correct program recall for \emph{Real-PyPI} is not available as the dataset only contains faulty programs.

In general, the recall is improved when the neural bug detector is trained on the filtered dataset (observed in 9/10 cases) up to $2.75\%$. This improvement indicates that the removal of type-related bugs from the training data enables the neural bug detectors to focus more on other non-type-related bugs. On the other hand, the precision is also reduced in 8 out of 10 cases. However, the change is generally smaller, with a maximum decrease of $-1.47\%$. We hypothesize that this decrease may be attributed to the oversampling strategy we used, rather than generating entirely new synthetic samples.


When assessing the \fbeta{} score, we evaluate both cases of $\beta=1$ (F-1) and $\beta=1.5$. When using the F-1 score, where recall is equally important as precision, filtering out type-related bugs from the training data does not yield a visible improvement in overall performance, as indicated by a better F-1 score in only 5 out of 10 cases. This finding aligns with our observation in \autoref{sec:influence-type-check} that integrating with type checkers is not beneficial in these cases.


When prioritizing bug identification ($\beta=1.5$), we note that the filtered dataset consistently outperforms the full dataset in all cases for the synthetic dataset. This observation suggests that the reduction in precision is less pronounced compared to the increase in recall when emphasizing bug detection over minimizing false alarms. This improvement extends to the real-world dataset as well, with the filtered dataset outperforming the full dataset in 3 out of 5 cases, while performing similarly in the case of GGNN. The slight variation in results for the real-world dataset may stem from the distribution shift between synthetic and real-world bugs.

% \todo{Size effect for each column}

% \begin{table*}[tb]
%     \centering
%     \caption{Performance change of detectors trained with full dataset and filtered dataset. Numbers are in percentage. Numbers after the dashed line show the relative change in performance. In general, filtering type-related bugs in training improves the localization accuracy but decreases the correct program recall.}
%     \begin{tabular}{|c|c:cc:c|c:cc:c|cc:c|}
%     \hline
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{Synthetic} & \multicolumn{4}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
%     \cline{2-12}
%     & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR}& \textbf{LA} & $\Delta$\\
%     \hline
%     CodeBert      & 95.94 $\rightarrow$ 95.54 & -0.42 & 92.90 $\rightarrow$ 93.23 & 0.36 & 95.61 $\rightarrow$ 95.31 & -0.32 & 35.33 $\rightarrow$ 35.43 &  0.27 & -- & 33.42 $\rightarrow$ 32.35 & -3.20 \\
%     GraphCodeBert & 96.27 $\rightarrow$ 95.90 & -0.38 & 93.82 $\rightarrow$ 94.01 & 0.20 & 96.09 $\rightarrow$ 95.63 & -0.48 & 36.50 $\rightarrow$ 39.21 &  7.43 & -- & 33.29 $\rightarrow$ 36.63 &  10.04 \\
%     UnixCoder     & 96.23 $\rightarrow$ 95.83 & -0.42 & 93.70 $\rightarrow$ 93.98 & 0.30 & 96.05 $\rightarrow$ 95.51 & -0.57 & 36.27 $\rightarrow$ 38.48 &  6.08 & -- & 33.29 $\rightarrow$ 35.89 &  7.81 \\
%     GGNN          & 92.97 $\rightarrow$ 92.74 & -0.25 & 72.64 $\rightarrow$ 73.30 & 0.91 & 92.64 $\rightarrow$ 92.16 & -0.51 & 14.76 $\rightarrow$ 14.67 & -0.63 & -- & 15.18 $\rightarrow$ 15.76 &  3.88 \\
%     GREAT         & 90.56 $\rightarrow$ 91.07 &  0.56 & 81.51 $\rightarrow$ 81.88 & 0.45 & 88.96 $\rightarrow$ 89.43 &  0.52 & 20.89 $\rightarrow$ 21.82 &  4.44 & -- & 20.94 $\rightarrow$ 23.06 &  10.11 \\
%     \hhline{============}
%     Average & \multicolumn{2}{r}{-0.18} & \multicolumn{2}{r|}{0.44} & \multicolumn{2}{r}{-0.27} & \multicolumn{2}{r|}{3.52} & -- & \multicolumn{2}{r|}{5.73}\\
%     \hline
%     \end{tabular}
    
%     \label{tab:impact-training} 
% \end{table*}

% \begin{table*}[tb]
%     \centering
%     \caption{Performance change of model trained with dataset excluding type-related bugs compared to the full synthetic dataset. A positive value means an improvement from the training with the full dataset}
%     \begin{tabular}{|c|c|c|c||c|c|c||c|c|c|}
%     \hline
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c||}{Synthetic 1} & \multicolumn{3}{c||}{Synthetic 2} & \multicolumn{3}{c|}{Real} \\
%     \cline{2-10}
%     & \textbf{CPR} & \textbf{LA} & \textbf{Joint} & \textbf{CPR} & \textbf{LA} & \textbf{Joint} & \textbf{CPR} & \textbf{LA} & \textbf{Joint}\\
%     \hline
%     CodeBert & -0.45 &  0.38 & -0.10 & -0.04 &  0.05 &  0.00 & -0.31 &  0.10 & -0.29 \\
%     GraphCodeBert & -0.47 &  0.39 & -0.10 &  0.06 &  0.43 &  0.22 & -0.46 &  2.71 & -0.37 \\
%     UnixCoder & -0.32 &  0.32 & -0.04 & -0.31 &  0.62 &  0.11 & -0.55 &  2.20 & -0.46 \\
%     GGNN & -0.28 &  0.62 &  0.13 & -0.49 & -1.83 & -1.15 & -0.29 &  0.18 & -0.27 \\
%     GREAT &  0.71 &  0.27 &  0.51 &  0.36 & -1.64 & -0.63 & 0.43 &  1.39 &  0.48 \\
%     Transformer & -3.88 & -1.99 & -3.03 & -3.37 & -2.43 & -2.91 & -2.76 & -1.20 & -2.68 \\
%     \hline
%     \end{tabular}
    
%     \label{tab:type oversampling} 
% \end{table*}

% \todo{Add rq headers to other parts}
\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
    \textbf{RQ4}: Removing type-related errors from the training dataset causes a significant increase in recall. Although a decrease in precision is also noted, the overall \fbeta{} score is improved in 8 out of 10 cases when $\beta=1.5$. 
    
    %In general, we observe that the performance of neural bug detectors trained without type-related bugs has a better localization accuracy (in 13/15 cases) while reducing the correct program recall (in 8/10 cases). This finding indicates that while type-related bugs diminish the detector's ability to localize bugs, they contribute positively to the detector's ability to decide if a program contains an error.
\end{tcolorbox}

==> initial-version/sections/existance.tex <==
\section{Existence of Type-Related Bugs}
\label{sec:existance}

This section summarizes why type checking is important to be used for detecting Python bugs, and examines the presence of type-related bugs in popular synthetic and real-world datasets. Additionally, it discusses the methodology for assessing the prevalence of type-related bugs in these datasets.


% It highlights the oversight of type checking in existing synthetic datasets and describes the process of identifying errors using the type checker. Additionally, it discusses the methodology for assessing the prevalence of type-related bugs in these datasets.


\subsection{Motivation}


% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=1\linewidth]{imgs/motivation.pdf}
%     \caption{The use of a neural bug detector in production}
%     \label{fig:motivation}
% \end{figure}

% Neural bug detectors focus on bug types (\textit{e.g.,} variable misuse) that traditional tools (\textit{e.g.,} type checkers) struggle to detect, and they are intended to complement these tools. \autoref{fig:motivation} illustrates the practical application of a neural bug detector in a real-world scenario, where developers employ a type checker alongside it. Firstly, the program undergoes type checking. If a bug is detected, it is promptly reported. If not, the program proceeds to the neural bug detector. If a bug is found, it is reported; otherwise, the program is deemed correct.

% When building a neural model, its use in production should be taken into consideration. Particularly, in this depicted scenario, it is important to note the following:

% \begin{tcolorbox}
% The neural bug detector is only run over programs for which the type checker does not detect a bug.
% \end{tcolorbox}

% Therefore, the training and evaluation of neural bug detectors should be performed with that statement in mind. In other words,
% \begin{itemize}
%     \item the model evaluation should respect the production setting \textit{i.e.,} the model should only be evaluated using bugs that cannot be caught by the type checker
%     \item the training of the model should maximize the performance of the model in production. That is, the final model should only focus on those bugs undetectable by the type checker and the training should be designed to achieve that.
% \end{itemize}

% However, in previous works, neither of these two items have been taken into account when building these neural models~\cite{xx,xx}. Therefore, in this paper, we evaluate previously proposed neural bug detectors under these practical circumstances ...

Previous work in creating neural bug detectors for Python has largely overlooked the potential presence of type-related bugs in their datasets due to the lack of type annotations in Python code. However, recent type checkers such as \texttt{pytype} \cite{pytype} based on \textit{type inference} can identify type-related bugs even in the absence of explicit type annotations. For example, in \autoref{lst:codeExp}, the variable usage \texttt{first} at line 8 can be detected by a type checker through type inference. In this context, \texttt{first} is expected to be a Boolean variable. Attempting member access for a boolean variable is invalid, resulting in an \textit{unsupported operand error} for the program.

In order to understand the influence of such defects on the performance of neural bug detectors, the first step is to assess the existence of such bugs in datasets used for training and evaluation. We evaluate existing synthetic and real-world bug detection datasets to address the following research question:

\begin{itemize}
   \item \textbf{RQ1:} \emph{How prevalent are type-related bugs in variable misuse datasets?}
\end{itemize}

%Synthetic datasets are commonly used for training bug-detection models due to the challenges associated with identifying specific types of bugs in real-world programs \cite{allamanis2017learning,hellendoorn2019global,VasicKMBS19}. Even in the existence of a dataset of real-world bugs, these datasets are typically either used as evaluation only or used in combination with synthetic bugs \cite{he2022distribution,allamanis2021self}. Typically, these synthetic faulty programs are derived from correct programs by replacing segments of the code to introduce specific types of bugs. In datasets tailored to dynamically typed programming languages, such as Python, the type consistency of the resulting faulty programs is generally disregarded. One reason for this oversight is that the original (correct) programs lack type annotations, hence Python type checkers that typically rely on using \textit{gradual typing} (such as \textit{mypy}\cite{mypy}) are unable to detect any type-related errors.   

%For example, a well-known synthetic dataset for Python variable misuse task ignores type consistency in the data generation process \cite{VasicKMBS19}. Moreover, subsequent research on the variable misuse task either directly uses this dataset \cite{RabinHA21,RabinHAH23,johnson2020learning} or generates synthetic datasets following a similar methodology \cite{kanade2020learning,pashakhanloo2022codetrek,troshin2022probing}. 

%However, type checkers such as pytype \cite{pytype} based on \textit{type inference} can identify type-related bugs in the source code even without explicit type annotations. \autoref{lst:codeExp} presents an example synthetic faulty program from the Python variable misuse dataset, where the variable usage \texttt{first} (colored in red) can be detected by a type checker through type inference. In this context, \texttt{first} is expected to be a boolean variable. Attempting member access for a boolean variable is invalid, resulting in an \textit{unsupported operand} error for the program.

% \todo{Find papers about using NNs in combination with traditional detection tools}
%While performing type checking is a common best practice for detecting type-related bugs early in the development cycle \cite{khan2021empirical, gao2017type}, synthetic bugs are also frequently used in training neural networks for automated bug detection. While neural bug detectors can identify a broader spectrum of bugs compared to type checkers, they typically focus on bugs that elude detection by traditional static analysis tools \cite{richter2022neural}. Consequently, the presence of type-related bugs in the dataset may influence the performance of the neural bug detectors. 

%To understand the prevalence of type-related bugs in the datasets used for training and evaluation, we conduct a study of existing synthetic and real-world bug detection datasets to address the following research question:

%\begin{itemize}
  %  \item \textbf{RQ1:} \emph{How prevalent are type-related bugs in the variable misuse datasets?}
%\end{itemize}

% the outcomes are typically perceived as less interpretable than those of type checkers, which have been extensively studied. Furthermore, type checkers are typically considered computationally more efficient than ML approaches, especially on large-scale projects. As we continue to integrate these ML-based tools for early bug detection, it is crucial to comprehend how these new tools should interact with traditional, well-established methods of bug detection to offer a comprehensive range of detention capabilities and interpretability.  

% To realize this vision, the first crucial question to address is how bugs detectable by traditional methods, such as type checkers, impact the performance of ML-based detectors. 


% \todo{Add caption to the listing and continue the example}
 
\subsection{Evaluation setup}
In this section, we present our methodology for conducting type checks on datasets designed for Python variable misuse bug detection. We detail the datasets used in our study and provide an overview of our approach.

\subsubsection{Datasets}
We analyze two widely used synthetic Python variable bug detection datasets and two real-world datasets. 


\textbf{ETH Py-150 synthetic bugs (\synthetic{})} \cite{hellendoorn2019global} is a dataset specifically crafted for the detection and correction of variable misuse bugs within Python functions. This dataset is synthetically generated from the ETH Python-150 dataset \cite{kanade2020learning} by substituting correct variable usages with incorrect ones, chosen randomly within the same function. For each faulty function, the dataset specifies the bug's location, a list of candidate variables for repair, and the correct variable in the candidates. The dataset contains 1.7M training functions, 200k for validation, and 950k for evaluation. 
% Given that the dataset's primary focus is on variable misuse bugs, it is apparent that a type checker would be able to detect a subset of these errors. For example, it could identify the incorrect usage of variable \texttt{first} as demonstrated in \autoref{lst:codeExp}.

\textbf{Synthetic training set (\synthetictwo{})} \cite{he2022distribution} is a training dataset constructed following a similar approach as \synthetic{}. Instead of directly creating synthetic bugs from the programs in the ETH Py150 dataset, this dataset is generated by extracting programs directly from the open-source projects used to construct Py150. Specifically, repositories without a commit fix related to real-world variable misuse bugs are used. In total, around 147k samples were constructed for both faulty and correct functions from 2654 repositories. 


\textbf{Py150 Real Bugs (\realpy{})} \cite{he2022distribution} is a dataset containing real variable misuse bugs extracted from open-source Python projects used to construct the Py150 dataset by applying a set of heuristics to identify commits fixing these bugs. However, the amount of faulty programs is insufficient to train a neural bug detector. We include the correct programs from the test splits as well as faulty programs from all splits. In total, the dataset contains 1,292 bugs and 61,539 correct programs

% Such bugs often need to be used together with synthetic bugs for training purposes \cite{he2022distribution}. Thus, we only use this dataset for evaluation and combine all bugs from train, validation, and test splits into a single set. 

% We use this dataset to evaluate the generalization of the neural bug detector trained on the synthetic dataset to real-world bugs.

\textbf{PyPI Real Bugs (\realpypi{})} \cite{allamanis2021self} contains 2436 faulty functions with different types of bugs found in all 285k packages from the Python Package Index (PyPI). We only filter out the variable misuse bugs from this dataset and use them for evaluation. Furthermore, this dataset is provided as commits to the fix of the bug. We use the provided information to extract original faulty programs from the source control of the projects. While some projects used in the dataset were deleted or renamed, we are able to extract 1,051 samples of variable misuse bugs from this dataset.


% \textbf{Swap Operands Detection (SWOP)} \cite{kanade2020learning} is a dataset aiming at detecting errors resulting from the erroneous swapping of operands of non-commutative operands. This dataset is also synthetically generated from the ETH Python-150 dataset by randomly swapping the operands of a single non-commutative operation within the code. The objective is to predict the presence of this bug within a function, making it a binary classification problem. The dataset contains 240k training examples, 30k validation examples, and 130k evaluation examples. Notably, certain error types in this dataset can also be identified by a type checker when the operator is defined for two types in a specific order. For example, the operator \texttt{\%} is defined for string formatting when a string is on the left-hand side and an integer is on the right-hand side. Inverting the position of these types makes the operator undefined, leading to a type checking error. 

\subsection{Addressing the RQ}
For each faulty code snippet in the datasets, we use \texttt{pytype} \cite{pytype} to detect type-related bugs within the function. Preprocessing and filtering are performed to ensure the bugs caught by the type checker are indeed the variable misuse bugs of interest. \autoref{fig:bug-label} shows an overview of the process.

%Since type checkers may also identify issues in the function other than the ones intended in the function \cite{rak2020python}, we only type check functions with bugs. Furthermore, preprocessing and filtering are performed to ensure the bugs caught by the type checker are indeed the variable misuse bugs of interest. \autoref{fig:bug-label} shows an overview of the process.

% Since type checkers may raise false positives due to their strict nature \cite{rak2020python}, we only type check functions with bugs.  we only consider faulty examples and use preprocessing to mitigate potential false positives. \autoref{fig:bug-label} shows an overview of the process.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/existance/bug_label.pdf}
    \caption{An overview of the process of labeling type-related bugs}
    \label{fig:bug-label}
\end{figure}

\textbf{Preprocessing:}
Given that each code snippet within the datasets only contains one function and omits the imported packages for that function, it is possible that the type checker may detect undesired \textit{import errors}. To mitigate such issues, our approach includes a dual-phase of type checking. Initially, the first phase of type checking is conducted to identify any absent packages. Subsequently, all detected missing packages are imported at the beginning of the code snippet.

\textbf{Type checking and filtering:}
Then a second phase of type checking is executed. To account for potential irrelevant issues raised by the type checker, we ignore all errors related to imported packages and internal errors from \texttt{pytype} such as \textit{pyi errors} indicating that \texttt{pytype} cannot produce type inference for the program. Finally, only errors detected on the same line as the variable misuse bug location are considered identifiable by the type checker. 
% for the \textit{VarMisuse} dataset, we only consider errors detected on the same line as the variable misuse location. For the \textit{SWOP} dataset, only \textit{unsupported operand} errors, the only type of bug in the dataset, are included. 

We conduct type checking on both the training and evaluation split across both datasets, quantifying the proportion of bugs identifiable by a type checker. We refer to these bugs identifiable by a type checker as \textit{type-related bugs}.

\subsection{Results}
\begin{table}[tb]
    \centering
    \caption{Percentage of type-related bugs within the training and evaluation splits of the datasets (\%).}
    \label{tab:existance}
    \begin{tabular}{ccc}
    \hline
      \textsc{Dataset}   & \textsc{Training} & \textsc{Evaluation}  \\
     \hline
     \synthetic{}& 19.56 & 19.52\\
     
     \synthetictwo{} & 14.45 & N.A. \\
     
     \realpy{} & N.A. & 5.72  \\
     
     \realpypi{} & N.A. & 4.00 \\ 
     \hline
    \end{tabular}

\end{table}

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/existance/error_types}
    \caption{Distribution of type-related bugs in the synthetic (top) and real-world (bottom) datasets. In \synthetic{}, we plot only the distribution of the evaluation split; the training split follows a similar distribution.}
    \label{fig:error-type}
\end{figure}

\autoref{tab:existance} shows the percentage of bugs detectable by a type checker within the training and evaluation sets of all four datasets. \autoref{fig:error-type} offers a more detailed analysis of type-related errors, illustrating the distribution of such bugs in both synthetic and real-world datasets. In general, there are five types of bugs that appear most frequently in the datasets:

\begin{itemize}
    \item \textit{name-error} (56.7\%-81.9\%) often arises when a variable name is used without prior declaration or in parallel with the declaration. For example, the definition and use of a variable are in different branches of an if-else statement.
    \item \textit{attribute-error} (12.9\%-30.9\%) occurs when an attribute is accessed on a variable that does not have that attribute. For example, accessing an attribute of an integer variable.
    \item \textit{unsupported-operand} (2.36\%-7.14\%) is raised when an unsupported operation is performed on variables. For example, attempting to add a string to an integer.
    \item \textit{wrong-arg-types} (1.93\%-6.76\%) is raised when a function is called with arguments of wrong types. This is typically related to a built-in function while type annotation exists, such as using \texttt{len} to access the length of an integer.
    \item \textit{not-writable} (3.36\% in \synthetictwo{} only) is raised when trying to modify an immutable variable, such as an immutable tuple.
    %a variable is used in a context that requires a writable variable,
    % e.g., attempting to modify an immutable tuple.
\end{itemize}

Most type-related bugs are linked to trivial errors, \textit{e.g.,} undefined variables in \emph{name-errors}. Consequently, neural models may excel in handling these instances, potentially inflating overall performance metrics. This poses a significant threat to evaluation, as these bugs may never be analyzed by the neural bug detectors if a type checker is incorporated. This problem is notably more significant in \synthetic{}, where roughly 20\% of the evaluation split comprises type-related bugs.%, whereas it is less prominent in real datasets where the proportions of such bugs are lower ($\sim$5\% and $\sim$4\% for Real-Py150 and Real-PyPI, respectively).

A significant portion of the training splits (approximately 20\% in \synthetic{} and 15\% in \synthetictwo{}) also comprises type-related bugs. This could potentially lead neural bug detectors to deviate their focus towards these bugs, which is undesirable in cases where developers use type checkers.


%Given the balanced nature of the synthetic datasets \textbf{Synthetic 1} and \textbf{Synthetic 2} (same percentage of correct and erroneous samples), the proportion of type-related bugs across the entire dataset equals approximately half the percentage noted in the table. 
%Notably, both synthetic datasets exhibit over 10\% of bugs identifiable by a type checker, with the training set of Synthetic 1 at 19.56\% and that of Synthetic 2 at 14.45\%, indicating a significant amount. 

%Real-world programs also tend to contain some type-related bugs, but the proportion is significantly lower than in synthetic datasets (5.27\% and 4.00\% for \textbf{Real-Py150} and \textbf{Real-PyPI}, respectively). 
%Thus, a neural bug detector trained on synthetic datasets may be biased toward type-related bugs, which are less prevalent in real-world scenarios. 
%The existence of type-related bugs in real-world datasets also highlights the importance of type checking for dynamically typed languages. 

% The similarity in percentage between training and evaluation sets may stem from the synthetic generation process of the Synthetic 1 datasets. At the same time, the real-world dataset \textbf{VarMisuse-Real} contains a significantly lower proportion of type-related bugs at 5.72\%. Thus, model trained on synthetic datasets may be biased towards type-related bugs, which are less prevalent in real-world scenarios.



%Compared to real-world datasets, the Synthetic 1 dataset contains a more significant portion of bugs categorized as \textit{name errors}, arising when a variable name is used without prior declaration. Such trivial bugs could potentially affect the performance of neural networks trained and evaluated on these datasets. 

%The distribution of type-related bugs in the Synthetic 1 dataset is similar to the two datasets, while Synthetic 2 contains a type of bug (not-writable) that is not observed in the real-world dataset. Furthermore, Synthetic 1 has notably more training samples compared to the evaluation set. We use Synthetic 1 as the main dataset for training in the following experiments.


\begin{tcolorbox}[left=1mm,right=1mm,top=1mm,bottom=1mm]
\textbf{RQ1}: A significant fraction of bugs in the evaluation dataset are detectable by a type checker, with more than half of these associated with trivial errors like undefined variables. Such occurrences may inflate performance metrics. Furthermore, the training dataset also includes a notable amount of type-related bugs, potentially impacting the focus of the neural bug detectors toward these bugs.

% A considerable proportion of bugs within the evaluation splits are of the type-related category. Over half of the type-related bugs are associated with trivial errors such as undefined variables, which bug samples could potentially inflate  performance evaluation. Furthermore, the training splits also contain a notable proportion of type-related bugs. This amount can potentially shift the focus of neural bug detectors towards these bugs, which is undesirable especially when developers use a type checker.
\end{tcolorbox}

==> initial-version/sections/intro.tex <==
\section{Introduction}

%\textbf{Context.}
% \todo{Papers on using NN together with type checker}
Bug detection is a crucial task in software engineering (SE). Studies suggest that between 0.5 to 25 bugs may occur may occur per 1000 lines of industrial code~\cite{mcconnell2004code,habib2018many}. The implications of these bugs in software systems can be profound, leading to outcomes ranging from minor system malfunctions to potential loss of human lives~\cite{fonseca2017empirical,jemal2022presence,poulsen2004software,zhivich2009real}.
Bug detection is even more important in dynamically typed languages such as Python and Javascript, which are more error-prone than statically typed languages~\cite{ray2014large}. Furthermore, the absence of mandatory type checking in these languages often leads to more type-related bugs compared to statically typed languages~\cite{gao2017type,khan2021empirical}. 
% Additionally, many bugs can remain hidden within the code for an extended period. For instance, it is estimated that, on average, it takes about 240 days to discover and fix a simple bug in a Java project~\cite{mosolygo2021rise}. Such hidden bugs in programs can result in severe consequences, ranging from minor system malfunctions to potential loss of human life\cite{fonseca2017empirical,jemal2022presence,poulsen2004software,zhivich2009real}. 

Automated bug detection aims to identify bugs early in the software development cycle. Traditionally, this task has been depending on static analysis which interprets the semantics of the source code \cite{aftandilian2012building,calcagno2015moving,hovemeyer2004finding}. Recent advances in machine learning (ML) have increased interest in using neural networks for identifying various bugs by learning implicit bug patterns from faulty programs \cite{habib2019neural}. These bug detectors typically aim to identify bugs, such as variable misuse~\cite{allamanis2017learning} or binary operator bugs~\cite{troshin2022probing}, in syntactically correct programs. Consequently, their training and evaluation datasets comprise both correct and faulty programs that are syntactically valid. 

% Consequently, they are complementary tools to be used alongside these traditional analyzers~\cite{richter2022neural}.

%Type checker is a type of static analysis tools that targets to identify bugs in the program based on types of variables. For static type languages such as C\#, Java and C++, type checking is integrated as a step in the compilation. However, for dynamically typed languages such as Python, type checking is performed by external tools. \todo{connect type checking with neural networks}

% \todo{Some more connections are needed}
% Recent advances in machine learning (ML) have sparked increased interest in using neural networks to identify a variety of bugs without the need for explicitly defining bug patterns~\cite{habib2019neural}. These neural bug detectors typically target to address bug types that elude traditional rule-based static analyzers (e.g., variable misuse~\cite{allamanis2017learning} or binary operator bugs~\cite{troshin2022probing}). Consequently, they are complementary tools to be used alongside these traditional analyzers~\cite{richter2022neural}.

%\textbf{Problem statement.}
% In SE practice, neural bug detectors are often used together with static analyzers like type checkers, as the latter is typically already integrated into the development environment. 

In statically typed languages, such as Java and C\#, type checking is integrated into the compiler's program analysis process. Hence, previous research on neural bug detectors for these languages has considered this aspect \cite{allamanis2017learning}. \autoref{fig:motivation} shows the use of a neural bug detector for a statically typed language where developers use a type checker in conjunction with the neural bug detector. The process begins with type checking; if a bug is identified by the type checker (categorized as \emph{type-related bug} in our paper), 
it is immediately reported and rectified. When the type checker does not find any bugs, the neural bug detector evaluates the program. It reports any discovered bugs, otherwise the program is deemed correct. Hence, \emph{neural bug detectors focus on programs for which the type checker does not detect any bugs}.

% In statically typed languages like Java and c\#, type checking is typically a part of the syntax checking process in the compiler. Thus, previous work on neural bug detectors for these languages has taken this factor into account \cite{allamanis2017learning}. \autoref{fig:motivation} illustrates the practical application of a neural bug detector for a statically typed language, where developers use a type checker alongside it. Firstly, the program undergoes type checking. If a type-related bug is detected, it is promptly reported and fixed. Otherwise, the program is checked by the neural bug detector. If a bug is found, it is reported; otherwise, the program is deemed correct. As a result, \emph{a neural bug detector only checks programs for which no bugs were detected by the type checker}.

\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{imgs/motivation.pdf}
    \caption{The use of a neural bug detector for statically typed languages}
    \label{fig:motivation}
\end{figure}

% Neural bug detectors focus on bug types (\textit{e.g.,} variable misuse) that traditional tools (\textit{e.g.,} type checkers) struggle to detect, and they are intended to complement these tools. 

%When building a neural model, its use in production should be taken into consideration. Particularly, in this depicted scenario, it is important to note the following:

%\begin{tcolorbox}
%The neural bug detector only checks programs for which the type checker does not detect a bug.
%\end{tcolorbox}

Thus, the training and evaluation of neural bug detectors must be contextualized to ensure their relevance and efficiency.
%\begin{itemize}
    %\item 
First, neural bug detector models should be evaluated exclusively on bugs not detectable by the type checker to ascertain their true effectiveness.
    %\item 
Moreover, the training of neural bug detectors should prioritize real-world performance to identify bugs that elude type checkers, thus enhancing their usefulness.

    %and the training should be designed to achieve that.
%\end{itemize}

% However, in previous works, neither of these two items have been taken into account when building these neural models~\cite{xx,xx}. Therefore, in this paper, we evaluate previously proposed neural bug detectors under these practical circumstances ...

% \todo{The problem does not raise for statically programming languages. Syntactically incorrectness}
% Such practice is commonly considered in neural bug detectors designed for statically typed languages such as C\#, where type checker is integrated into the compiler \cite{allamanis2017learning}.

However, when studying neural bug detectors for dynamically typed languages, such as Python, previous research often disregards this crucial aspect due to the absence of inherent static type checkers~\cite{VasicKMBS19,kanade2020learning,hellendoorn2019global}. As a result, little is known about the impact of type checking on the performance of these neural bug detectors.
%these detectors are assessed on bugs that are potentially detectable by a type checker. 
Nonetheless, the growing popularity of optional type annotations in these languages, which facilitate static type checking, suggests a shift towards integrating type checking in the development workflow \cite{khan2021empirical,di2022evolution}. When a type checker is used, for example, as part of continuous integration, existing performance assessments may not accurately represent the neural network's effectiveness in such settings. Moreover, training detectors on such bugs may inadvertently skew the model's detection capability towards less relevant types. 

%In this paper, we study \emph{how neural bug detector performs in a practical setting} while a static type checker is used during the development process and a set of bugs are already caught by the type checker.



%\textbf{Objectives.}

This paper explores the impact of type checking on 
%the training and evaluation of 
contemporary neural bug detectors in the context of Python, a widely used dynamically typed language. Our analysis encompasses a broad spectrum of neural architectures, including Gated Graph Neural Networks (GGNN) \cite{li2015gated}, GREAT \cite{hellendoorn2019global}, CodeBERT~\cite{feng2020codebert}, GraphCodeBERT~\cite{guo2020graphcodebert}, and UnixCoder~\cite{guo2022unixcoder}. 
Our study investigates variable misuse bugs, which are frequently targeted by neural bug detectors.
We assess how type-related bugs influence the training and evaluation of neural bug detectors using both synthetic and real-world datasets. 
%we identify type-related bugs within both synthetic and real-world datasets, leveraging these datasets to assess how type-related bugs influence the training and evaluation of neural bug detectors. 
More specifically, we address the following research questions:


\noindent \textbf{RQ1:} \emph{How prevalent are type-related bugs in variable misuse datasets?}

\noindent \underline{Motivation}:
Before examining how type checking influences the training and evaluation of neural bug detectors, it is imperative to assess if bugs identifiable by a type checker exist within popular variable misuse datasets.

% As neural bug detectors are often used together with traditional type checkers in SE practice, 
% %integrated into continuous integration pipelines.  Hence, 
% neural bug detectors primarily aim to identify bugs that elude detection by type checkers. The presence of type errors in the dataset may influence the performance of the neural bug detectors. Therefore, it is crucial to understand the prevalence of type-related bugs in the datasets used for training and evaluation.

\noindent \underline{Results}: We find that a significant proportion of bugs in synthetic datasets (up to 19.56\%) can be identified by a type checker. This is significantly higher than the proportion of type-related bugs in real-world datasets (up to 5.72\%). %The portion of easily detectable synthetic bugs may even be higher if type annotations are actively used in the programs. 

\noindent \textbf{RQ2:} \emph{How does type checking influence the performance of neural bug detectors when they are used together?}

\noindent \underline{Motivation}: 
Given that existing datasets pertaining to the variable misuse task contain a notable proportion of type-related bugs identified by a type checker, the aim of RQ2 is to evaluate how effective it is to use neural bug detectors together with a type checker in terms of performance.

\noindent \underline{Results}: 
We find that incorporating a type checker enhances the performance of GGNN and GREAT. Using a type checker with the other neural networks results in an increased recall (more bugs detected) but decreased precision (more false alarms). Therefore, for those neural bug detectors, the decision to use a type checker depends on the practical significance of recall versus precision.


%We find that using that using a type checker in conjunction with neural bug detectors improves recall while reduces precision. The decision to use a type checker hinges on the practical significance of recall versus precision. Generally, a type checker is used when the priority is bug detection over the minimization of false positives.

\noindent \textbf{RQ3:} \emph{How do type-related bugs influence the performance evaluation of neural bug detectors?}

\noindent \underline{Motivation}: 
When incorporating a type checker into the development process, neural bug detectors should prioritize detecting bugs that elude type checkers. Hence, understanding their effectiveness in identifying this category of bugs is crucial.
% Furthermore, many of the type-related bugs identified in the synthetic datasets are related to trivial errors such as undefined variables, which may potentially be easier to detect. Therefore, we investigate the performance of the neural bug detectors on type-related bugs and compare it with other types of bugs.% in this research question.

\noindent \underline{Results}: We observe that neural bug detectors exhibit notably better performance in type-related bugs. 

%removing type-related errors reduces the performance of neural bug detectors for \emph{all} aspects. This discrepancy significantly influences the overall performance of neural bug detectors, leading to inflated evaluation results.

%The difference can be as high as 34.71\%. Consequently, removing type-related bugs generally reduces the performance of neural bug detectors (up to 5.61\%) despite their small portion in the dataset. Such finding indicates that the evaluation of the neural bug detectors may be overly optimistic.

\noindent \textbf{RQ4:} \emph{How do type-related bugs influence the training of neural bug detectors?}

\noindent \underline{Motivation}: Since neural bug detectors tend to perform better on type-related bugs, the existence of such bugs in the training data may bias the neural model towards the wrong type of bugs already caught by the type checker. Therefore, in RQ4, we investigate how filtering out type-related bugs impacts the training of neural bug detectors.

\noindent \underline{Results}: We find that neural bug detectors trained on programs excluding type-related bugs perform better in identifying bugs beyond the scope of type checkers on synthetic and real-world datasets. We also observe a decrease in the precision of bug detection. An improvement in joint performance is observed when the emphasis is on bug identification. 

% the improvement in recall is generally more significant than the decrease in precision, leading to an improvement in joint performance.

% when deciding if a program contains bug (correct program recall). However, the improvement in localization accuracy is more significant than the decrease in the correct program recall. 

% Hence, in a practical SE scenario with the combined use of type checkers and neural bug detectors, programs containing type-related bugs should be removed from training set.


% Such finding indicates that the inclusion of type-related bugs in the training data depends on the purpose of the neural bug detectors.


%\todo{citation}
%To explore the the effect of type-related bugs, We focus on the most popular bug detection task focused by neural bug detectors: variable misuse. We experiment with two neural network architectures, including graph neural networks and transformer, and two training paradigms: full training and fine-tuning. We train these models with one synthetic dataset as previous work and evaluate them on two synthetic and one real world dataset. 

% Our empirical results demonstrate that a significant portion of synthetic defects in Python can be caught by a type checker. We also present the impact of these type-related defects in both the training and evaluation phases of ML models for defect detection and how this may influence the practicability of the ML models trained with these samples. Specifically, this work makes the following contribution to the software engineering research:

% \begin{enumerate}
%     \item We show a substantial number of synthetic defects in two Python defect detection datasets can be identified by a type checker.
%     \item We reveal the effect of type checking on evaluations, highlighting that GNNs and LLMs perform better at identifying type-related defects over others, which may cause evaluation to be overly optimistic. 
%     \item We discuss the impact of type-related defects on ML training, considering both standard training approaches and fine-tuning, for both GNN and LLM architectures. 
% \end{enumerate}

% %\textbf{Implications.}
% Our findings underscore the significance of conducting a systematic evaluation of neural bug detectors within practical contexts, rather than depending solely on aggregated metrics. Through analyzing the performance disparities between type-related and other categories of bugs, researchers and practitioners are afforded more detailed understanding of a detector's capabilities. This analysis enables the informed selection of the most appropriate neural network architecture tailored to the specific bug types encountered in real-world scenarios. Moreover, we emphasize the critical role of curating training data, particularly when type checkers are integrated into the development workflow. In such cases, it is imperative to exclude programs containing type-related bugs from the training dataset.

\noindent\textbf{Added value.} Our findings offer practical insights into the optimal use of a type checker with a neural bug detector for dynamically typed languages, particularly when prioritizing bug identification over minimizing false alarms. Integrating a type checker with a neural bug detector necessitates excluding type-related bugs from evaluation to mitigate the potential of overly optimistic results. Likewise, during training, it is advisable to exclude these bugs to improve bug detection. 

\noindent\textbf{Artifacts.} Artifacts for this study are available online~\cite{artifacts_icse25}.

\noindent \textbf{Organization.}
This paper is organized as follows: \autoref{sec:background} introduces the background and context of our study. Following this, \autoref{sec:existance} examines the prevalence of type-related bugs in popular datasets for variable misuse. \autoref{sec:effect} evaluates the impact of type checking on the training and evaluation of neural bug detectors. Subsequently, \autoref{sec:discusssion} explores the potential implications of our findings. Finally, \autoref{sec:rel-work} reviews related literature, and \autoref{sec:conclusion} concludes the paper. 
% Our findings provide practical insights into when a type checker should be used together with a neural bug detector for dynamically typed languages, specifically, when bug identification is more important compared to avoiding false alarms. When a type checker is integrated with the neural bug detector, the exclusion of type-related bugs from the evaluation data is necessary to prevent potential over-optimistic performance. Moreover, during training, it is advisable to omit these bugs to enhance bug identification.  Artifacts for this study are available at \cite{?} 

% Our findings underscore the significance of conducting a systematic evaluation of neural bug detectors within practical contexts, rather than depending solely on aggregated metrics. Integrating a type checker into the development process necessitates the exclusion of type-related bugs from the evaluation split to prevent the inflation of performance metrics. Moreover, during training, it is advisable to omit these types to enhance localization accuracy. Artifacts for this study are available at \cite{?} \todo{Anomalized Repo and organization}
% \todo[inline]{paragraph summarizing all sections is missing}

% Additionally, we highlight how different defect types affect training outcomes and provide recommendations for data collection strategies.


==> initial-version/sections/rel-work.tex <==
\section{Related Work}
\label{sec:rel-work}

\subsection{Neural bug detectors}

\paragraph{Target bug types}

Multiple studies have shown the effectiveness of using neural networks for bug detection. Besides variable misuse bugs studied in this paper, neural networks have been used to detect other types of bugs, such as operand swapping \cite{troshin2022probing}, wrong binary operator \cite{troshin2022probing,he2022distribution,allamanis2021self}, and identifying wrong argument or return values of a function \cite{allamanis2021self,li2020deep}. Most of the work adapts the strategy of joint learning of detection and repair of the program together~\cite{VasicKMBS19}.

\paragraph{Proposed models}

The predominant models utilized for bug detection can be broadly categorized into Transformers, GNNs, and hybrid methods~\cite{hellendoorn2019global}. Transformers process programs as sequences of tokens, with the flexibility of being either trained from scratch~\cite{hellendoorn2019global} or fine-tuned (\textit{e.g.,} CuBERT~\cite{kanade2020learning}, CodeBERT~\cite{feng2020codebert}, GraphCodeBERT~\cite{guo2020graphcodebert}, UnixCoder~\cite{guo2022unixcoder}, etc.). GNN models, on the other hand, interpret programs in the form of graphs featuring diverse edges such as control flow, data flow, etc.~\cite{allamanis2017learning}. Hybrid approaches combine both models. For example, GREAT~\cite{hellendoorn2019global} combines the transformer architecture with edge types from the program graph. The sandwich model~\cite{hellendoorn2019global} alternates between transformer layers and graph neural layers, forming a cohesive approach.

This paper explores a range of models including CodeBERT, GraphCodeBERT, UnixCoder, GGNN, and GREAT, thereby encompassing the entire spectrum of commonly employed approaches for bug detection.

\paragraph{Datasets}
Due to the lack of real-world bugs, training on real-world bugs alone is typically not sufficient to obtain a high-performing bug detector \cite{he2022distribution,richter2023train}. As a result, many approaches have been focused on generating synthetic bugs. The most common approach is to randomly perturb a program with a set of predefined mutation rules \cite{allamanis2017learning,VasicKMBS19}.

Recent work demonstrates that neural detectors trained on synthetic bugs do not perform well on real-world bugs \cite{allamanis2022graph}. This difference in performance can be attributed to the different characteristics between synthetic and real-world bugs \cite{alrashedy2023learning,he2022distribution}. As a result, many studies have experimented with mixing synthetic and real-world bugs in training \cite{he2022distribution,richter2023train}.

At the same time, other approaches attempt to generate synthetic datasets that are more similar to real-world bugs. For example, Richter et al. \cite{richter2022learning} use a learning based approach to generate faulty programs taking the context of the original program into account. SemSeed \cite{patra2021semantic} extracts a set of bug patterns from real-world bugs and applies the pattern most similar to the original program to generate a synthetic bug.

Our study takes a different perspective on analyzing the datasets for training neural bug detectors. Specifically, we investigate how type-checking influences the performance of these detectors and offer recommendations to enhance their practicality when deployed in such scenarios.


%In this work, we focus on another aspect of the neural bug detectors: whether they pass the type checker. We study the impact of type checking on the performance of these detectors and provide suggestions on how to make them more practical. 

% \subsection{Synthetic bug generation}


\subsection{Combining static analysis and neural networks}
Static analysis has long been used to enhance the performance of neural networks used on code. In neural bug detectors, static analysis generates a program graph used as input to the neural network \cite{allamanis2017learning,hellendoorn2019global}. When repairing the bug, feedback generated from the compiler is used as additional information to help the neural network \cite{yasunaga2020graph,ye2022selfapr,tarlow2020learning}.

Another task commonly associated with static analysis is type inference. When employing a neural network for variable type prediction, particularly in dynamically typed languages, the predicted types often lack guarantees of consistency with the type checker \cite{cassano2023type,allamanis2020typilus,yee2023machine}. In such scenarios, a type checker is used to (1) guide the search space of types and (2) ensure the coherence of the predicted types \cite{pradel2020typewriter,cassano2023type,wei2022typet5,pandi2020opttyper}.

In this work, we show how and when a type checker should be used together with a neural bug detector to improve the overall bug detection performance. Furthermore, we show how bugs detectable by a type checker can influence the training and evaluation of neural bug detectors.

% \todo[inline]{A section about empirical study with type checker?}

==> sections/evaluation.tex <==
\section{Effect of Type Checking}

\subsection{Motivation}


%Though type-related errors exist in both synthetic and real-world datasets, the former contains a much higher proportion of such bugs. 

In scenarios where a type checker is employed, neural bug detectors are expected to focus on bugs not detectable by the type checker. Thus, to offer recommendations for deploying neural bug detectors alongside a type checker, it's crucial to comprehend the impact of type-related bugs on the training and testing of these neural systems. As a result, we aim to address the following two research questions:


%In real world setting when a type checker is deployed in development, the type-related bugs are often caught before by the type checker 

%they are pushed into the code base by a type checker. Thus, it is important to understand how type-related errors influence the training and testing of the the neural bug detectors. Specifically, we investigate the following two research questions:

%This section presents our experiment results demonstrating the effect of type-related bugs on the performance of these neural bug detectors in both evaluation and training. Specifically, we investigate the following two research questions:

\begin{itemize}
    \item \textbf{RQ2:} How do type-related bugs influence the evaluation of neural bug detectors?
    \item \textbf{RQ3:} How do type-related bugs influence the training of neural bug detectors?
\end{itemize}


\subsection{Experiment Setup}
In this section, we introduce the neural networks used in the neural bug detectors in our experiments. This is followed by datasets and evaluation metrics we used to investigate the research questions. 


\begin{table}[tb]
    \centering
    \caption{Bug Detection Neural Networks}
    \begin{tabular}{cccc}
    \hline
    \textsc{Model} & \textsc{Architecture} & \textsc{Training strategy} \\
    \hline
    GGNN \cite{allamanis2017learning} & GNN & From scratch \\
    % \hline
    % 6-layer transformer \cite{hellendoorn2019global} & Transformer & Full \\

    CodeBERT \cite{feng2020codebert} & Transformer & Fine-tuning \\

    GraphCodeBERT \cite{guo2020graphcodebert} & Transformer & Fine-tuning \\

    UnixCoder \cite{guo2022unixcoder} & Transformer & Fine-tuning \\

    GREAT \cite{hellendoorn2019global} & Hybrid & From scratch \\
    \hline
    \end{tabular}
    \label{tab:models}
\end{table}

\subsubsection{Neural bug detectors}


The first column of \autoref{tab:models} displays the neural bug detectors utilized in our experiments. The second column of the same table illustrates the architectures corresponding to each considered model. We cover three widely employed architectures: transformers, GNNs, and hybrid methods. Lastly, the third column denotes whether the model is trained from scratch (\textit{i.e.,} initialized with random weights) or fine-tuned (\textit{i.e.,} initialized with a pre-trained checkpoint).

%In this paper, we focus on three main architectures of neural networks: graph neural networks, transformers, and hybrid methods. Furthermore, they can also be categorized by the training strategy: full training or fine-tuning. \autoref{tab:models} presents the neural networks used in our experiments.

%When fine-tuning a pre-trained model, we follow previous work \cite{troshin2022probing} by appending a classification layer to the pre-trained model and fine-tuning the entire model. For the full training models, we adapt the implementation from previous work \cite{hellendoorn2019global}

\subsubsection{Datasets}


We adopt the methodology established in prior studies concerning training with a synthetic dataset and assessed using both the synthetic test split from the same dataset and real-world datasets~\cite{hellendoorn2019global,habib2019neural,he2022distribution,richter2023train}. Specifically, we select the Synthetic 1 dataset as our training dataset because of its larger volume of data.
%For detecting variable misuse task, we use the training split of the \textit{Synthetic 1} due to its larger amount of data and its distribution of type-related errors is closely aligned with that of real-world scenarios. Subsequently, we evaluate the trained models also on the test split of the dataset.

The trained neural bug detectors are also evaluated in the real world in both real-world datasets: \emph{Real-Py150} and \emph{Real-PyPI}. For the \emph{Real-Py150} dataset, we include the correct programs from the test splits as well as faulty programs from all splits. All processed variable misuse bugs from \emph{Real-PyPI} dataset are also included in the evaluation. 

%\textbf{Data leakage check}
Since the real-world datasets are constructed independently from the \emph{Synthetic 1} dataset, some of the real-world bug programs may also appear in the training set of \emph{Synthetic 1}. To avoid such data leakage issues, all potential duplicated samples are excluded from the datasets from evaluation. Specifically, we use the metadata of each sample as a heuristic and remove all program samples that are from the same file in the same repository and have the same function signature as any samples from the synthetic training set. \todo[inline]{how many are removed - does the number of real bugs stated earlier include the duplicates?}

% We perform data leakage check on the \textit{VarMisuseReal} dataset and found it does not contain any files from the repositories as the synthetic dataset. Thus, we include all faulty programs from this dataset and randomly sample the same number of correct programs to build a balanced real world test set.

\subsubsection{Metrics}
Following previous work \cite{hellendoorn2019global,habib2019neural}, we use separate metrics for bug classification and localization. First, we measure the \textit{correct program recall} (\textbf{CPR}), which is the recall of a neural bug detector in deciding that a program is free from any bugs. Specifically, given a neural bug detector and a set of \emph{correct} programs $\mathcal{P}_c$, the \textbf{CPR} is defined as:
\begin{equation*}
    CPR(\mathfrak{D}, \mathcal{P}_c) = \frac{|\{p\in\mathcal{P}_c|d_{\mathfrak{D}(p)} = \texttt{false}\}|}{|\mathcal{P}_c|}
\end{equation*}
where $d_{\mathfrak{D}(p)}$ represents the decision of the neural bug detector on the program.

Then, for all the faulty programs, we measure the \textit{location accuracy} (\textbf{LA}) which is the proportion of programs where the model correctly identifies the location of the bug. Let $\mathcal{P}_f$ represent the set of \emph{faulty} programs and $l_p$ represent the location of the bug for the program $p$, \textbf{LA} is defined as follows.
\begin{equation*}
    LA(\mathfrak{D}, \mathcal{P}_f) = \frac{|\{p\in\mathcal{P}_f|d_{\mathfrak{D}(p)} = \texttt{true} \land l_{\mathfrak{D}(p)} = l_p\}|}{|\mathcal{P}_f|}
\end{equation*}
where $l_{\mathfrak{D}(p)}$ represent the bug location of the faulty program $p$ predicted by the neural bug detector.

\chadded{
Finally, to measure the differences in performance of the two settings, we use \emph{ratio change}. Given the performance values of two settings $p_a$ and $p_b$, the ratio change $\Delta$ of $p_b$ with respect to $p_a$ is calculated as follows:
}
\begin{equation*}
    \Delta = \frac{p_b - p_a}{p_a} \times 100
\end{equation*}
\subsubsection{Training settings}
Previous work often trains the neural bug detector with the joint training objective of both bug detection and repair \cite{VasicKMBS19,allamanis2017learning,hellendoorn2019global}. In our preliminary experimentation, we notice that training without the repairing loss results in either similar or degraded performance compared to the joint objective. Consequently, we opt to utilize the joint training objective, as done in previous studies.

When training GGNN and GREAT models, we use the same hyperparameter configurations as in previous work~\cite{hellendoorn2019global} and train for 5 and 10 epochs, respectively. For fine-tuning, we train each model for 1 epoch and use a learning rate of 0.00001 with a linear learning rate scheduler.

\subsection{RQ2: Evaluation on type-related bugs}
\subsubsection{\todo[inline]{for RQ1, we have these four sections: Motivation, Setup, Approach, and Results. therefore, this should be called Approach to be consistent}Addressing the RQ}
In this section, we evaluate the performance of neural bug detectors on type-related bugs compared to other bugs when trained with a synthetic dataset on the variable misuse task. We divide the evaluation dataset into two groups based on the type checking results in the evaluation samples: type-related bugs and other bugs. We then evaluate the performance of the neural networks on these two groups separately. Furthermore, we measure the impact of the type-related bugs on the overall performance by evaluating all faulty programs and faulty programs filtering type-related ones. We only include the location accuracy as the focus of this experiment is on faulty programs. 

% When performing full training on the models, we use the same hyperparameter configurations as in \cite{hellendoorn2019global} and train for 5, 10 and 12 epochs respectively. For fine-tuning, we train each model for 1 epoch and use a learning rate of 0.00001 with a learning rate scheduler.

% \begin{table*}[tb]
%     \centering
%     \caption{Location Accuracy on all bugs, type-related Bugs, other bugs and the difference between type-related bugs and other bugs for synthetic and real world datasets. The numbers are in percentage.}
%     \begin{tabular}{|c|c|c|c|c||c|c|c|c||c|c|c|c|}
%     \hline
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c||}{Synthetic 1} & \multicolumn{4}{c||}{Synthetic 2} & \multicolumn{4}{c|}{Real} \\
%     \cline{2-13}
%     & \textbf{All} & \textbf{Type Bug} & \textbf{Other bugs} & \textbf{Diff} & \textbf{All} & \textbf{Type Bug} & \textbf{Other bugs} & \textbf{Diff} & \textbf{All} & \textbf{Type Bug} & \textbf{Other bugs} & \textbf{Diff}\\
%     \hline
%     CodeBert & 93.95 & 99.07 & 92.72 & 6.34 & 77.17 & 86.37 & 75.78 & 10.59 & 35.40 & 36.36 & 35.33 & 1.03\\
%     \hline
%     GraphCodeBert & 94.74 & 99.18 & 93.68 & 5.50 & 81.14 & 91.13 & 79.64 & 11.49 & 36.58 & 37.88 & 36.50 & 1.38\\
%     \hline
%     UnixCoder & 94.74 & 99.49 & 93.61 & 5.88 & 74.85 & 85.60 & 73.22 & 12.38 & 36.32 & 37.14 & 36.27 & 0.87\\
%     \hline
%     GGNN & 76.41 & 93.47 & 72.43 & 21.04 & 44.99 & 44.75 & 45.01 & -0.26 & 15.05 & 19.67 & 14.79 & 4.88\\
%     \hline
%     GREAT & 84.31 & 97.00 & 81.34 & 15.65 & 51.26 & 50.87 & 51.29 & -0.43 & 20.73 & 24.59 & 20.52 & 4.07\\
%     \hline
%     Transformer & 67.22 & 75.38 & 65.31 & 10.07 & 41.79 & 40.77 & 41.87 & -1.09 & 8.84 &  9.84 & 8.78 & 1.06 \\
%     \hline
%     \end{tabular}
    
%     \label{tab:location-accuracy}
% \end{table*}

\begin{table*}[tb]
    \centering
    \caption{Location accuracy on type-related bugs and other bugs for synthetic and real-world datasets. The numbers are in percentage. We observe that the neural bug detectors perform better on type-related bugs compared to other bugs in all cases.}
    \begin{tabular}{|c|cc|cc|cc|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{Synthetic} & \multicolumn{2}{c|}{Real-Py150} & \multicolumn{2}{c|}{Real-PyPI} \\
    \cline{2-7}
    & \textbf{Type} & \textbf{Other} & \textbf{Type} & \textbf{Other} & \textbf{Type} & \textbf{Other}\\
    \hline
    CodeBert      & 99.07 & 92.90 & 36.36 & 35.33 & 60.00 & 33.42\\
    GraphCodeBert & 99.34 & 93.78 & 37.88 & 36.50 & 68.00 & 33.29\\
    UnixCoder     & 99.41 & 93.70 & 37.14 & 36.27 & 56.67 & 33.29\\
    GGNN          & 94.07 & 72.64 & 21.43 & 14.76 & 23.68 & 15.18\\
    GREAT         & 97.24 & 81.51 & 28.57 & 20.89 & 50.00 & 20.94\\
    \hline
    \end{tabular}
    
    \label{tab:la-bug-types}
\end{table*}

\begin{table*}[tb]
    \centering
    \caption{Impact of filtering type-related bugs on overall location accuracy. Numbers are in percentage. Type-related bugs make the model performance over-optimistic.}
    \begin{tabular}{|c|ccc|ccc|ccc|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{Synthetic} & \multicolumn{3}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
    \cline{2-10}
    & \textbf{Full} & \textbf{Filtered} & $\Delta$ & \textbf{Full} & \textbf{Filtered} & $\Delta$ & \textbf{Full} & \textbf{Filtered} &$\Delta$\\
    \hline
    CodeBert      & 94.11 & 92.90 & -1.29 & 35.40 & 35.33 & -0.17 & 34.28 & 33.42 & -2.51\\
    GraphCodeBert & 94.91 & 93.82 & -1.15 & 36.58 & 36.50 & -0.23 & 34.41 & 33.29 & -3.26\\
    UnixCoder     & 94.82 & 93.70 & -1.18 & 36.32 & 36.27 & -0.14 & 34.13 & 33.29 & -2.45\\
    GGNN          & 76.78 & 72.64 & -5.39 & 15.17 & 14.76 & -2.68 & 15.54 & 15.18 & -2.34\\
    GREAT         & 84.55 & 81.51 & -3.59 & 21.36 & 20.89 & -2.19 & 22.18 & 20.94 & -5.61\\
    \hline
    \end{tabular}
    
    \label{tab:la-impact}
\end{table*}


\todo{CPR is not mentioned for this research question before}
\begin{table*}[tb]
    \centering
    \caption{Performance of the bug detection pipeline shown in \autoref{fig:motivation}. $\Delta$ shows the percentage change w.r.t. the Full performance in \autoref{tab:la-impact}. The pipeline provides notable improvement to bug localization while marginally reducing correct program recall.\todo[inline]{i don't understand the figures in this table}}
    \begin{tabular}{|c|c:cc:c|cc:c|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
    \cline{2-8}
    & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR} & \textbf{LA} &$\Delta$\\
    \hline
    CodeBert      & 94.15 & -1.55 & 39.22 & 10.80 & -- & 35.58 & 3.77 \\
    GraphCodeBert & 94.61 & -1.55 & 40.31 & 10.20 & -- & 35.45 & 3.01 \\
    UnixCoder     & 94.57 & -1.54 & 40.12 & 10.45 & -- & 35.68 & 4.55 \\
    GGNN          & 91.28 & -1.49 & 19.97 & 31.61 & -- & 18.81 & 21.01 \\
    GREAT         & 87.67 & -1.49 & 25.72 & 20.41 & -- & 24.32 & 9.64 \\
    \hline
    \end{tabular}
    
    \label{tab:pipeline}
\end{table*}

\subsubsection{Results}
\autoref{tab:la-bug-types} shows the location accuracy of the neural bug detectors on type-related bugs (\textbf{Type}) and other bugs (\textbf{Other}) across synthetic and real-world datasets. 


Comparing the performance of the neural bug detectors on synthetic and real-world datasets, we observe that these detectors perform much better on the synthetic datasets compared to the real-world bugs, consistent with previous work~\cite{he2022distribution,allamanis2021self}. This discrepancy can be attributed to the distribution shift between synthetic and real-world bugs~\cite{he2022distribution}. 

Neural bug detectors consistently perform better in identifying type-related bugs, with a difference reaching up to 34.71\% for GraphCodeBert within the \emph{Real-PyPI} dataset. This finding aligns with our observations from the previous research question regarding the trivial nature of type-related bugs.

%indicates that neural bug detectors are indeed better at identifying type-related bugs with are composed of a large portion of trivial errors as shown in \autoref{fig:error-type} 

To check the influence of type-related bugs on the overall performance, \autoref{tab:la-impact} shows the impact of filtering type-related bugs on the overall location accuracy. The ratio of change in the filtered dataset compared to the full dataset is also noted in the table ($\Delta$). Since all neural bug detectors perform better on type-related bugs, we observe that the removal of type-related bugs generally reduces the performance of the neural bug detectors. The highest reduction is observed in the \emph{Real-PyPI} dataset, where the removal of type-related bugs results in a reduction of up to 5.61\% for the GREAT model, even though the type-related bugs only constitute 4\% of the dataset.

%In general, models using a full training strategy tends to bias more towards type-related bugs compared to fine-tuning models. This can be explained by fine-tuning models are already pre-trained with a large amount of code data and thus are less likely to be influenced by the type-related bugs in the training data. At the same time, the impact of type-related bugs on the performance also varies across different datasets, with the highest impact observed in the \emph{Real-PyPI} dataset and the lowest in the \emph{Real-Py150} dataset.

\chadded{
Our observations indicate that, despite being comparatively more effective than other bug types, the performance of neural bug detectors for identifying type-related bugs in real-world datasets remains suboptimal. Therefore, integrating neural bug detectors with a type checker within the pipeline as depicted in \autoref{fig:motivation}, is expected to enhance the performance in bug localization. To evaluate the performance of this integrated pipeline, we conducted experiments using the type checker on the correct programs within the \emph{Real-Py150} dataset. 
}

\chadded{
Given that a type checker can identify a broad range of issues beyond variable misuse, we adopt the filtering approach similar to that described in \autoref{fig:bug-label}, focusing exclusively on the subset of type-related bugs appeared in the distribution observed for variable misuse errors (\autoref{fig:error-type}). This approach resulted in the type checker achieving a \textbf{CPR} of 98.46\%. \autoref{tab:pipeline} shows the performance of the bug detection pipeline in \autoref{fig:motivation}. The pipeline provides a notable improvement to bug localization while marginally reducing correct program recall. We suspect that the reduction in correct program recall is due to the type checker and the neural bug detectors tending to raise false alarms on different programs.
}

\begin{tcolorbox}
\textbf{RQ2}: 
Our findings reveal that bug detectors exhibit superior performance in detecting type-related bugs compared to other types of bugs. The removal of these bugs from the evaluation dataset leads to a reduction in bug localization accuracy by up to 5.61\%. This suggests that the inclusion of type-related bugs in the evaluation dataset, particularly when utilizing a type checker, may yield overly optimistic evaluation results.

% Irrespective of the training paradigm or model architecture, our observations indicate that neural bug detectors consistently exhibit better performance on type-related bugs compared to other bugs. Additionally, despite type-related bugs constituting less than $20\%$ of the dataset, their removal results in a reduction of up to $5.61\%$ in the detector's bug localization accuracy. This suggests that type-related bugs are relatively easier to identify for neural bug detectors trained on synthetic datasets. Consequently, the presence of type-related bugs in the evaluation dataset may lead to overly optimistic evaluation results.

\end{tcolorbox}


\subsection{RQ3: Effect of type-related bugs on training}

\subsubsection{Addressing the RQ}
In this section, we investigate the impact of filtering type-related bugs from the training data on the performance of the neural bug detectors. Neural bug detectors trained with the \emph{full dataset} are compared with those trained with the \emph{filtered dataset} using both correct program recall and location accuracy on all samples from the evaluation datasets.

%\textbf{Training Dataset Preparation}
A naive approach to filter type-related bugs from the training data is to remove all samples that are identified as type-related bugs. However, this approach may result in a significant reduction in the size of the training data as well as an imbalance in the correct and faulty programs. To mitigate these issues, we \textit{replace} the type-related bugs with other bugs in the training data by randomly oversampling other bugs in the dataset. This approach ensures that the size of the training data remains the same and the balance between correct and faulty programs is maintained.

%\textbf{Evaluation}
\todo[inline]{move the paragraph "We target..." to the 2nd in this section}We target to measure the practical performance of neural bug detectors in a real-world setting where a type checker is integrated in the development process. Thus, we only focus on bugs that are beyond the scope of type checkers and filter all type-related bugs from the evaluation datasets. 

\subsubsection{Results}

The performance change of neural bug detectors trained with full dataset and filtered dataset is shown in \autoref{tab:impact-training}. Values on the left side of the arrow show the performance of the full training dataset while the right side represents the performance of filtered training. The numbers after the dashed line show the relative change in performance of the two versions of training datasets. Correct program recall for \emph{Real-PyPI} is not available as the dataset only contains faulty programs.

In general, the localization accuracy experiences enhancement when the neural bug detector is trained on the filtered dataset, as observed in 13 out of 15 cases. This enhancement is particularly prominent in real-world datasets, with average increases of $3.52\%$ and $5.73\%$ for Real-Py150 and Real-PyPI, respectively. This improvement can be attributed to the elimination of type-related bugs from the training data, enabling the neural bug detectors to concentrate more on detecting other types of bugs beyond the limitations of a type checker.

%The improvement can be as high as 10.11\% for the GraphCodeBert in the \emph{Real-PyPI} dataset. Such improvement can be explained by the removal of type-related bugs from the training data, which allows the neural bug detectors to focus more on other types of bugs beyond the scope of a type checker. Moreover, the performance gain is generally more significant in the real world datasets compared to the synthetic datasets. This improvement means that the filtering dataset is generally more effective in practical settings.

Additionally, we also note a decrease in correct program recall in 8 out of 10 cases. However, this reduction is considerably less notable compared to the enhancement in localization accuracy. Specifically,  the average change ratio for \textbf{LA} is about $2.44\times$ the average change ratio for \textbf{CPR} in the synthetic datasets and $13.04\times$ in the \textit{Real-Py150} dataset. We hypothesize that this phenomenon may be attributed to the oversampling strategy we employed, rather than generating entirely new synthetic samples.

%Nevertheless, a decrease in the correct program recall is also observed for a significant number of cases (8/10), though the decrease is generally less significant compared to the improvement in the localization accuracy. 

%The highest decrease is observed in the \emph{Real-Py150} dataset, where the correct program recall decreases by 0.57\% for UnixCoder. We suspect such a decrease is not statistically significant and is likely due to the random sampling during the replacement of type-related bugs in the training data.

%\chadded{
%Comparing the impact of training on the filtered dataset on \textbf{CPR} and \textbf{LA}, we observe that the impact on \textbf{LA} is much more significant than the impact on \textbf{CPR}. The average change ratio for \textbf{LA} is about $2.44\times$ the average change ratio for \textbf{CPR} in the synthetic datasets and $13.04\times$ in the \textit{Real-Py150} dataset. Such observation confirms that the removal of type-related bugs from the training data generally provides more improvement than the decrease in correct program recall.
%}

% To measure the statistic significance of the performance change, we perform Wilcoxon signed-rank test on the performance change of the neural bug detectors. When checking the significance of the performance change in \textbf{CPR} with alternative hypothesis that the mean of performance change is less than zero, a p-value of 0.14 is obtained, indicating that the performance change is not statistically significant. However, when checking the significance in \textbf{LA} with alternative hypothesis that the mean of performance change is greater than zero, a p-value of 0.003 is obtained, indicating that the performance change is statistically significant.

% Furthermore, we also calculate the effect size pf the Wilcoxon signed-rank test of the performance change for each dataset, which is shown in the last row of \autoref{tab:impact-training}. The effect size is calculated using the formula $r = Z/\sqrt{N}$, where $Z$ is the z-score of the test and $N$ is the number of samples. Similarly, we observe that the effect size of the performance change in \textbf{LA} is generally larger than the effect size of the performance change in \textbf{CPR}, indicating that the performance change in \textbf{LA} is more significant.


 
% \todo{Size effect for each column}
\begin{table*}[tb]
    \centering
    \caption{Performance change of detectors trained with full dataset and filtered dataset. Numbers are in percentage. Numbers after the dashed line show the relative change in performance. In general, filtering type-related bugs in training improves the localization accuracy but decreases the correct program recall.}
    \begin{tabular}{|c|c:cc:c|c:cc:c|cc:c|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{Synthetic} & \multicolumn{4}{c|}{Real-Py150} & \multicolumn{3}{c|}{Real-PyPI} \\
    \cline{2-12}
    & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR} & $\Delta$ & \textbf{LA} & $\Delta$ & \textbf{CPR}& \textbf{LA} & $\Delta$\\
    \hline
    CodeBert      & 95.94 $\rightarrow$ 95.54 & -0.42 & 92.90 $\rightarrow$ 93.23 & 0.36 & 95.61 $\rightarrow$ 95.31 & -0.32 & 35.33 $\rightarrow$ 35.43 &  0.27 & -- & 33.42 $\rightarrow$ 32.35 & -3.20 \\
    GraphCodeBert & 96.27 $\rightarrow$ 95.90 & -0.38 & 93.82 $\rightarrow$ 94.01 & 0.20 & 96.09 $\rightarrow$ 95.63 & -0.48 & 36.50 $\rightarrow$ 39.21 &  7.43 & -- & 33.29 $\rightarrow$ 36.63 &  10.04 \\
    UnixCoder     & 96.23 $\rightarrow$ 95.83 & -0.42 & 93.70 $\rightarrow$ 93.98 & 0.30 & 96.05 $\rightarrow$ 95.51 & -0.57 & 36.27 $\rightarrow$ 38.48 &  6.08 & -- & 33.29 $\rightarrow$ 35.89 &  7.81 \\
    GGNN          & 92.97 $\rightarrow$ 92.74 & -0.25 & 72.64 $\rightarrow$ 73.30 & 0.91 & 92.64 $\rightarrow$ 92.16 & -0.51 & 14.76 $\rightarrow$ 14.67 & -0.63 & -- & 15.18 $\rightarrow$ 15.76 &  3.88 \\
    GREAT         & 90.56 $\rightarrow$ 91.07 &  0.56 & 81.51 $\rightarrow$ 81.88 & 0.45 & 88.96 $\rightarrow$ 89.43 &  0.52 & 20.89 $\rightarrow$ 21.82 &  4.44 & -- & 20.94 $\rightarrow$ 23.06 &  10.11 \\
    \hhline{============}
    Average & \multicolumn{2}{r}{-0.18} & \multicolumn{2}{r|}{0.44} & \multicolumn{2}{r}{-0.27} & \multicolumn{2}{r|}{3.52} & -- & \multicolumn{2}{r|}{5.73}\\
    \hline
    \end{tabular}
    
    \label{tab:impact-training} 
\end{table*}

% \begin{table*}[tb]
%     \centering
%     \caption{Performance change of model trained with dataset excluding type-related bugs compared to the full synthetic dataset. A positive value means an improvement from the training with the full dataset}
%     \begin{tabular}{|c|c|c|c||c|c|c||c|c|c|}
%     \hline
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c||}{Synthetic 1} & \multicolumn{3}{c||}{Synthetic 2} & \multicolumn{3}{c|}{Real} \\
%     \cline{2-10}
%     & \textbf{CPR} & \textbf{LA} & \textbf{Joint} & \textbf{CPR} & \textbf{LA} & \textbf{Joint} & \textbf{CPR} & \textbf{LA} & \textbf{Joint}\\
%     \hline
%     CodeBert & -0.45 &  0.38 & -0.10 & -0.04 &  0.05 &  0.00 & -0.31 &  0.10 & -0.29 \\
%     GraphCodeBert & -0.47 &  0.39 & -0.10 &  0.06 &  0.43 &  0.22 & -0.46 &  2.71 & -0.37 \\
%     UnixCoder & -0.32 &  0.32 & -0.04 & -0.31 &  0.62 &  0.11 & -0.55 &  2.20 & -0.46 \\
%     GGNN & -0.28 &  0.62 &  0.13 & -0.49 & -1.83 & -1.15 & -0.29 &  0.18 & -0.27 \\
%     GREAT &  0.71 &  0.27 &  0.51 &  0.36 & -1.64 & -0.63 & 0.43 &  1.39 &  0.48 \\
%     Transformer & -3.88 & -1.99 & -3.03 & -3.37 & -2.43 & -2.91 & -2.76 & -1.20 & -2.68 \\
%     \hline
%     \end{tabular}
    
%     \label{tab:type oversampling} 
% \end{table*}

% \todo{Add rq headers to other parts}
\begin{tcolorbox}
    \textbf{RQ3}: Removing type-related errors from the training dataset causes a significant increase in localization accuracy. Although a decrease in correct program recall is also noted, it is substantially less significant.
    
    %In general, we observe that the performance of neural bug detectors trained without type-related bugs has a better localization accuracy (in 13/15 cases) while reducing the correct program recall (in 8/10 cases). This finding indicates that while type-related bugs diminish the detector's ability to localize bugs, they contribute positively to the detector's ability to decide if a program contains an error.
\end{tcolorbox}
